Clustering of bivariate satellite time series: a quantile approach

Clustering has received much attention in Statistics and Machine learning with the aim of developing statistical models and autonomous algorithms which are capable of acquiring information from raw data in order to perform exploratory analysis.Several techniques have been developed to cluster sampled univariate vectors only considering the average value over the whole period and as such they have not been able to explore fully the underlying distribution as well as other features of the data, especially in presence of structured time series. We propose a model-based clustering technique that is based on quantile regression permitting us to cluster bivariate time series at different quantile levels. We model the within cluster density using asymmetric Laplace distribution allowing us to take into account asymmetry in the distribution of the data. We evaluate the performance of the proposed technique through a simulation study. The method is then applied to cluster time series observed from Glob-colour satellite data related to trophic status indices with aim of evaluating their temporal dynamics in order to identify homogeneous areas, in terms of trophic status, in the Gulf of Gabes.

==> Bivariate Quantile Regression Clustering/data.tex <==
\section{Chl-a and KD-490 levels in the Gulf of Gabes}\label{sec2}
The Gulf of Gabes is a Mediterranean zone with important biological resources and rich coastal, marine and freshwater ecosystems. In the last decades the Gulf of Gabes reported several environmental problems mainly due to the presence of human activities associated with over-fishing and seabed trawling while the presence of chemical factories in the Sfax site resulting on a wide wastewater pollution \citep{Aloulou:2012,Rabaoui:2013,Zaghden:2014,Fourati:2018}.
The results had led  to  several issues as the local appearance of red tides \citep{hamza:1994} as well as the changes or decline of the distribution of some marine species \citep{el:2016,el:2018}.

The European Community indicates  the diffuse Chlorophyll type-a (Chl-a) concentrations as a trophic status indicator of the sea-water. High Chl-a levels may lead to hypoxic or anoxic events.  KD-490 indicates how the solar light can penetrate to deeper water and can be used to evaluate the potential disturbance to the water ecosystem.

In this work, we considered two datasets comprising the Chl-a concentrations and the KD-490 levels made available by ACRI (\texttt{hermes.acri.fr}) in the framework of the GlobColour Project (\texttt{www.globcolour.info}).
The datasets were formed by monthly values of Chl-a concentrations and KD-490 levels in the Gulf of Gabes from January, 2003 to December, 2011 for a total of $108$ time-points.
Data were obtained by calibrating Ocean Colour data provided by different satellite missions, such as MERIS, SeaWiFS and MODIS. For each month, gridded data with 1.8-km resolution are available and  a  grid of $4,033$ points  covers the entire Gulf of Gabes.

%%%decribe the tow figures 
In Figure \ref{fig:1} we report the average levels of Chl-a concentration and KD-490 index for all the sites.
% describe the temporal trend of the selected sites.
%%%%%%%%%%%%%%%

\begin{figure}
	\centering
	\begin{tabular}{cc}
		\includegraphics[width=0.5\linewidth]{meanChla_trim.png}  &
		\includegraphics[width=0.5\linewidth]{meanKD490_trim.png} \\
		%(a) & (b)
	\end{tabular}
	\caption{Observed grid-points (4033 sites) in the Gulf of Gabes for Chl-a (left) and KD-490 (right) and two example sites reported in Figure \ref{fig:2}.}\label{fig:1}
\end{figure}
The highest average levels of Chl-a and KD-490 were reported near the coastal area, in the north-eastern zone (Sfax) and in the southern part (Djerba) of the Gulf. The spatial distribution of the average values between Chl-a and KD-490 appears to have a similar spatial and temporal behaviour, but not everywhere. In fact as shown in Figure \ref{fig:2} the example site 1 exhibits a strong seasonal pattern both in the Chl-a and KD-490 indicators, with a strong correlation between the two time series (Pearson $\rho$: 66.1\%); in the second example site 2 there is a clear difference between the trend of the Chl-a concentration with respect to the KD-490 one as attested by a weak correlation (Pearson $\rho$: 30.7\%).

\begin{figure}
	\centering
	\begin{tabular}{cc}
		\includegraphics[width=0.5\textwidth]{example1.png}  &
		\includegraphics[width=0.5\textwidth]{example2.png} \\
		(1) Lat: 10.88; Long: 33.99 & (2) Lat: 11.08; Long: 34.86
	\end{tabular}
	\caption{Temporal trend of Chl-a and Kd-490 in the two selected example sites.}\label{fig:2}
\end{figure}

The dataset is affected by outliers due to measurement errors  (Chl-a concentration lower than 0.05 $mg/m^{-3}$: 1.0\%; KD-490 levels lower than 0.05 $m^{-1}$: 2.8\%) and by a  different amount of missing observations
% please verify how many observations are missing
(Chl-a: 19.1\%; KD-490: 1.8\%).

The presented dataset presents several features which makes the clustering task challenging: a strong seasonality and a high variability,  the presence of outliers and a non bell-shaped distribution. The proposed classification may help to assess the trophic status of this area combining the information provided by different temporal Chl-a and KD-490 levels.


==> Bivariate Quantile Regression Clustering/discussion.tex <==
\section{Discussion}\label{sec6}
In this paper we have proposed a new model based clustering technique,  that is capable of handling asymmetric clusters with presence of outliers as well as considering different quantile levels of the observed data. Our clustering strategy is based on the finite mixture model theory where each component of the mixture of AL distributions, which constitutes of the density of bivariate random variables which are potentially correlated, is assumed to represent a cluster with the skewness parameter of AL distribution being used to directly model the quantiles of interest. Our proposed technique therefore adds on to the richness of the recent burgeoning of non-Gaussian approaches to model-based clustering.

As the AL distribution provides a direct link between the maximum likelihood theory and minimization of a quantile regression check loss function \citep[see][]{koenker1999goodness,yu2001bayesian}, we estimate the cluster specific  parameters, which are the parameters of the mixing AL distribution, through a Bayesian quantile regression approach. Following from \cite{Waldmann2015} we implement our bivariate clustering model that is based on Bayesian bivariate quantile regression. We note that due to the dependence in the constructed likelihood for the bivariate random variables there are no closed form available conditional posteriors for the model parameters. We therefore, introduce MH steps to estimate the parameters through MCMC.

In our simulation experiment we considered three clusters two of which are not distinctively different from each other. However, an evaluation of the power of our proposed algorithm in reconstructing the three groups indicates a good performance with respect to the other competitive methods. We have applied the procedure to time series observed from GlobColour data related to Chlorophyll type-a concentrations and KD-490 levels in order to identify homogeneous areas in the Gulf of Gabes with respect to the temporal behavior of these water indicators. We defined clusters that are similar by different combination of quantiles of the two indicators. It is important to note that as different choice of quantiles implies changes in the clustering, this method may be particularly suitable for defining areas at different risk when considering two indicators at different quantile levels. More particularly, important features are of absolute interest in environmental sciences and ecology. \citep{schmidt2012estimating}.

We note that both Chl-a concentrations and KD-490 levels are affected by several spatially varying factors. Therefore, a potential future development of this work is to model spatial dependence for the time series observed at different spatial sites. This could be achieved either through Markov random fields that considers the nearest neighbors \citep{Gaetan:2017,jiang2012clustering}. By borrowing information from neighboring observation sites, this could lead to more smooth clusters. Another possible extension is to perform clustering at multiple quantiles instead of fixing the levels of quantiles. However, caution has to be taken in this case to avoid the issue of crossing quantiles.


==> Bivariate Quantile Regression Clustering/introduction.tex <==
\section{Introduction}\label{sec1}

The European Community with the European Union Water Framework Directive 2000/60/EC (WFD) indicated a series of trophic status indicators with the scope to monitor the status of the sea-water in order to restore and protect water-bodies from further degradation \citep{directive2000european,Alikas:2015}. 
The light diffuse attenuation coefficient at 490 nm (KD-490) is an ecologically important water property that
provides information about the availability of light to underwater communities  which influences ecological
processes and biogeochemical cycles in natural waters \citep{Yang:2020}.
Together with KD-490, the Chlorophyll type-a (Chl-a) is commonly used as a proxy for phytoplankton biomass and as an indicator for eutrophication; high concentration levels may lead to hypoxic or anoxic events while low levels may result in improvement in water quality \citep{Dabuleviciene:2020}. The joint use of two complementary indices as the KD-490 and the Chl-a allows to take into account different aspects of water quality ranging from availability of light to underwater communities to the trophic status.

In this context, the classification of areas with a different level of impact may help Institutions to define a program of conservation and environmental protection. The European WFD 2000/60/EC set a series of rules to classify areas at different level of ``impact'' considering summary statistics (average, geometric mean, or percentile) of a single indicator over a predetermined temporal window (1 year, 5 years, etc, \ldots) with respect to a reference condition represented by no or very low human pressure \citep{poikane2010defining}. The definition of ``reference condition'' may be particularly complex and limited to each specific context \citep{Pardo:2012}. 

Measures of the KD-490 and Chl-a indices are obtained  from satellite sensors.
The use  of satellite data needs to consider aspects relative to unreliability for different reasons and mainly due to the presence of cloud contamination or malfunctioning of the sensor onboard the satellite; pre-processing procedures are often required to remove some site and measurements before using the data for the application \citep{alvera2012outlier,Stafoggia:2017}.

In this paper, we concentrate our efforts to overcome the classification based on simple summary statistics considering the temporal component in order to provide more reliable results since it takes into account the time dynamics of a water bodies indicator (i.e. seasonal behaviour, inter-annual variability, etc\ldots). 
In fact, standard clustering techniques %\citep{Ward:1963,MacQueen:1967} 
were often applied considering the summary statistics of the determinants of interest, and so, potentially valuable information about the temporal behaviours (e.g. trend, peaks, and seasonal patterns) is lost. 


In the environmental field time series clustering has gained popularity for grouping time series with similar temporal pattern %\citep{Liao2005} 
covering a wide series of applications and approaches \citep{Cazelles:2008,Giraldo:2012,shi2013remote,Finazzi:2015,Haggarty:2015,Gaetan:2017}.

 Moreover very often the summary statistics suffer from the lack of robustness in presence of contaminated data.
In this respect quantile regression appears attractive due to the possibility to overcome these pre-processing issues with the possibility of choosing a particular quantile of interest \citep{Barbosa:2011, Monteiro:2012}. 
Another juncture concerns that most of the published work considered the clustering of univariate response variable \citep{Barbosa:2011,Monteiro:2012} or even a different weight between average value and temporal trend \citep{li2016bivariate} while some other attempts were performed taking into account the joint distribution of two or more variables of interest or the joint modelling of more quantiles. \citep{gaetan2016clustering,Zhang:2019,Sottile:2019}.

Therefore we propose a Bayesian clustering technique to define groups of temporal patterns that are similar considering the quantile of interest on bivariate time series. More in detail, the application regards monthly time series of Chl-a concentrations and KD-490 levels, obtained by satellite data sensors over the Gulf of Gabes (Tunisia), a Mediterranean zone with important biological resources and rich coastal, marine, and freshwater ecosystems. Since the last few decades, due to fast and uncontrolled urbanization and industrialization, the Gulf of Gabes is experiencing an irreversible degradation of the local coastal area. \citep{ayadi:2015,el:2017}. 

The paper is organized as follows. The next section illustrates our data on Chl-a and KD490 on the Gulf of the Gabes. In Section 3 we introduce the Bayesian quantile regression with an extension to the bivariate case and proposing our clustering procedure. In Section 4 we present a simulation study for illustrating the performances and peculiarities of the procedure. Section 5 reports the results of the application to the Chlorophyll-a and KD-490 satellite data on the Gulf of the Gabes. In the last section  we discuss the relative strengths and weaknesses of our proposal.


==> Bivariate Quantile Regression Clustering/methods.tex <==
\section{Statistical modelling and inference}\label{sec3}
 \subsection{Multivariate quantile regression and asymmetric Laplace distribution}
We start by considering the  univariate case.
 Let $ Q_{p}(y|x) $, for $ 0<p<1 $, be the $p$-th quantile regression function of the univariate continuous random variable $ y $ given $ x$, a vector of  covariates.
 We suppose that $ Q_{p}(y|x)=x'\beta $, where $ \beta $ is a vector of unknown parameters to be estimated. Then a quantile regression model can be defined as $y=x'\beta+e$
where $ e$ is an error term  with  density function $f(\cdot;p) $ and  the $ p $-th quantile equal to zero, i.e. $ \int_{-\infty}^{0}f(e;p)de=p$.
Owing to the data $(y_t,x_t')$, $t=1,\ldots, T$, the  estimate of $\beta$ is classically \citep{koenker1978regression} obtained by minimizing 
\begin{eqnarray}\label{eq2}
	\hat{\beta}=\underset{\beta}{\text{argmin}}\sum_{t=1}^{T}\rho_{p}(y_{t}-x_{t}'\beta),
\end{eqnarray}
where $ \rho_{p}(\cdot) $ is the check loss function, i.e. $ \rho_{p}(z)=z(p-I(z<0)) $.

\citet{koenker1999goodness} showed that there is a direct relationship between minimizing (\ref{eq2}) and the maximum likelihood theory using independent variables $y_t$ with  Asymmetric Laplace   (AL) density
\begin{equation}
	f(e;p)=\frac{p(1-p)}{\sigma}\exp\left\{-\rho_{p}\left(\frac{e}{\sigma}\right)\right\},\label{eq3}
\end{equation}
where $ \sigma>0 $  is an additional   scale parameter.

In the following we will exploit the representation of $y$ with density \eqref{eq3} as a location scale mixture of Gaussian random variable  \citep{Kotz2001}, namely
\begin{eqnarray}
	y=x'\beta+\theta \sigma w+\omega \sigma\sqrt{ w}\,\nu \label{eq5}
\end{eqnarray}
where $ \nu\sim \mathcal{N}(0,1) $, and $ w $ is a exponential random variable with  $E(w)=1$. Here $\nu $ and $ w $ are mutually independent and
$\theta=(1-2p)/\{p(1-p)\}$ and $\omega^{2}=2/\{p(1-p)\}$.


The literature has focused on univariate response variable with only a few studies considering extension to multivariate case \citep{Benoit2012,Benoit2013,Waldmann2015,Petrella2019a}.


In particular \cite{Petrella2019a} considered a multivariate  asymmetric Laplace distribution \citep{Kotz2001} to specify a quantile regression model for the random vector
$\tilde{y}=(y_1,\ldots,y_q)'$ in the mixture representation
\begin{equation}
	\tilde{y}=X'\tilde{\beta}+ D\Theta {w} +\sqrt{w}D\Sigma^{1/2}\tilde{\nu} \label{eq3.20}
\end{equation}

Here  $\tilde{\nu}$ denotes a $q$-dimension standard Gaussian vector and $w$ is a exponential random variable with unit mean.
The matrix $X$ is a $q\times L$  regressor matrix and $\tilde\beta$ is a $L$-dimensional unknown vector. The other parameters of the model are contained in  $D = \operatorname{diag}(\tilde\sigma)$, with $\tilde{\sigma}=(\sigma_1,\ldots,\sigma_q)'$,  $\sigma_j>0$, $j=1,\ldots,q$  and $\Theta= \operatorname{diag}(\theta_1,\ldots,
\theta_q)'$ with $\theta_j = (1 - 2p_j)/[p_j (1 - p_j]$. 

Moreover the matrix $\Sigma=\Omega R(\tilde\phi)\Omega$ is a $q \times q$ positive definite matrix   with $R(\tilde\phi)$ being a correlation matrix, that depends on a vector of parameters $\tilde\phi$, and $\Omega= \operatorname{diag}(\omega_1^2,\ldots,\omega_q^2)$,
with entry $\omega_{j}^{2}={2}/[p_{j}(1-p_{j})]$. Note that using this formulation the component $y_j$ will  always be mutually dependent, even though $R(\phi)$ is an identity matrix.

In this paper we  consider a slight different approach with respect to  \eqref{eq3.20}.
We use the same idea as in \cite{Waldmann2015} and we set

\begin{equation}\label{eq:ald}
	\tilde{y}=X'\beta+ D\Theta \tilde{w} +{W}^{1/2}D\Sigma^{1/2}\tilde{\nu} 
\end{equation}
with $\tilde{w}= ({w}_1,\ldots,w_q)'$ and ${W}= \operatorname{diag}({w}_1,\ldots,{w}_q)$
allowing a different  exponential random variable with unit mean $ w_j$ for each component.


With this variation   model \eqref{eq:ald} does not define a proper multivariate asymmetric Laplace distribution as in \citet{Kotz2001}. However the model becomes more flexible and can cover the case of mutually independent components.
Now the challenge  lies in finding a multivariate density
for $\tilde{w}$, $	e(\tilde{w};\gamma)$, with marginal exponential distributions for the $w_j$ in order to guarantee that the marginal distributions for the response variables are still asymmetric Laplace. Here the parameter $\gamma$ is a generic dependence parameter.
%Therefore the multivariate density function of \eqref{eq:ald}
%\begin{eqnarray}
%	\textrm{ald}(\tilde{y}|\tilde{x},\beta,D,R(\phi),\gamma) 
%	&=&\int_{(0,\infty)^q} (2\pi)^{-q/2}|W^{{1}/{2}}\varSigma W^{{1}/{2}}|^{-{1}/{2}}\times \nonumber\\
%	&& \exp\left\{-\frac{1}{2}(\tilde{y}-X'\beta- D\Theta \tilde{w})'W^{-{1}/{2}}\varSigma^{-1}W^{-{1}/{2}}(
%	\tilde{y}-X'\beta- D\Theta \tilde{w})\right\}\times\nonumber\\
%	&& f(\tilde{w};\gamma)d\tilde{w}
%\end{eqnarray}

Several multivariate exponential distributions   have been proposed in the literature \citep[Ch. 47]{kotz:balakrishnan:johnson}.
\cite{Waldmann2015} adopt the simplest specification that the exponential variables are independent, i.e. $\gamma=0$.

In view of the bivariate real data example in this paper we exemplify our construction by using the bivariate density proposed by \cite{Downton1970}, namely
\begin{equation}\label{eq:downton}
	e(\tilde{w};\gamma)= \frac{1}{(1-\gamma)}\exp \left\{-\frac{1}{1-\gamma}\left(w_{1}+w_{2}\right)\right\}
I_{0}\left(\frac{2}{1-\gamma}\sqrt{\gamma w_{1}w_{2}}\right)
\end{equation}
where $ 0\le\gamma < 1 $
and $I_{0}(a)=\sum_{k=1}^{\infty}\frac{a^{2k}}{4^{k}(k!)^{2}}$ is the modified Bessel function of the first kind of order zero.
The value $\gamma$ represents the 
Pearson's product-moment correlation and $ \gamma=0 $ implies independence between the $w_1$ and $w_2$.
Coupling \eqref{eq:ald} with the density \eqref{eq:downton} we obtain a  flexible specification of a bivariate quantile regression model that covers the case of independence between  the components when $R(\phi)$ is an identity matrix and $\gamma=0$.




\subsection{Model-based clustering}\label{subsec:mixmod}
Suppose that we observe  data over $n$ statistical units and, for simplicity,  the same number $q\times T$  of values $y_{ijt}$,  $j=1,\ldots, q$, $t=1,\ldots,T$, for each statistical unit $i$, $i=1,\ldots,n$.
We collect the observations for each unit into the vector $\boldsymbol{y}_i = (\tilde{y}_{i1}',\ldots, \tilde{y}_{iT}')'$, with
$\tilde{y}_{it} = (y_{i1t},y_{i2t},\ldots y_{iqt})'$, $t=1,\ldots,T$.
The vectors  $\boldsymbol{y}_i$ are supposed to be independent.
The whole dataset will be denoted by $\mathcal{Y}=(\boldsymbol{y}_1,\ldots,\boldsymbol{y}_n)$.

Our statistical  problem is to cluster the $n$ statistical units, i.e. the sites,  into the clusters $\{1,\ldots,K\}$, $K\ll n$.
We follow a  mixture-model  approach \citep{mclachlan:peel:2000}  to clustering  according to which the cluster membership of the $i$th unit is represented by a latent random variable  ${c}_i \in \{1,\ldots,K\} $ , where $c_{i} = k$ indicates if the $i$-th units belongs to the cluster $k$. 

The memberships ${c}_i$, $i=1,\ldots,n$ are supposed independent and identically distributed  variables with 
$\Pr(c_{i} = k)=\alpha_k$, $ 0<\alpha_{k}<1 $, for all $k=1,\ldots,K$ and $ \sum_{k=1}^{K}\alpha_{k}=1 $.



Given the cluster membership,  $c_{i}$,  observations for the $i$-th unit are generated by the mixture model specified hierarchically, namely 

\noindent\textbf{the observation level}
\begin{equation}\label{eq:model}
		\tilde{y}_{it}|c_i,\tilde{w}_{it}\sim\mathcal{N}_q(X_{t}'\tilde\beta_{c_i}+ D_{c_i}\Theta \tilde{w}_{it},{W}_{it}D_{c_i}\Sigma_{c_i}D_{c_i}{W}_{it}), \qquad i=1,\ldots,n,\quad t=1,\ldots,T 
\end{equation}
		conditionally independent distributed, with $\Sigma_{c_i}=\Omega R(\phi_{c_i})\Omega$;

\noindent \textbf{the latent process level}
\begin{equation}
		\tilde{w}_{it}|c_i\sim e(w,\gamma_{c_i}), \quad i=1,\ldots,n,\quad t=1,\ldots,T
\end{equation}
		conditionally independent distributed
\begin{equation}
		c_i \sim \operatorname{Multinomial}(1,{\alpha}), \quad i=1,\ldots,n
\end{equation}
independent distributed.  


\subsection{Bayesian inference}\label{subsec:bayinf}
We adopt a Bayesian approach to make inference on the model parameters.
The inference is facilitated by the fact that the mixture model is  specified hierarchically. Moreover
the conjugacy of some priors leads to  updates with
simple and established methods for drawing from the full
conditional distribution.
%Moreover it is possible to get the posterior probability of membership of a single vector, $\Pr(c_i=\cdot|\mathcal{Y})$.


\noindent \textbf{Prior distributions}

A common choice for the prior distribution of $\alpha$ is $ {\alpha}\sim \mathcal{D}(a_{1},...,a_{K}) $, where $\mathcal{D}$ is the Dirichlet distribution with parameters $a_1, \ldots, a_K > 0$;  % which is a conjugate prior for the mixing proportions

The choice $ \tilde\beta_{k} \sim \mathcal{N}(b_k,P_k),\, k=1,\ldots,K$, identically and independent distributed is still common and simplifies the simulation. Setting $ b_k=0 $ and $ P_k=a\,I $, for $ a \gg 0 $, leads to an improper prior.
		
		 Specification of the  prior distributions for
		$\tilde\sigma_1,\ldots,\tilde\sigma_k$ and $\tilde\phi_1,\ldots,\tilde\phi_k$  is complicated  by the complex requirement that the matrices $D_k\Omega R(\phi_{k})\Omega D_k$ are  non-negative definite matrices.
We follow \citet{barnard:mcculloch:meng:2000} and   work  by specifying prior for variances  and correlation matrices.
For the variances we put the priors $ \sigma^2_{kj} \sim \mathrm{IG}(s_{k},d_{k}),\quad k=1,\ldots,K,\quad j=1,\ldots,q$,  identically and independent distributed,
	where $IG$ is  the inverse gamma distribution,
	with the shape $ s_{k}$  and $ d_{k}$ scale parameters.
	\citet{barnard:mcculloch:meng:2000} discussed the relative merits of choosing a prior for $\tilde\phi_1,\ldots,\tilde\phi_k$ independent from $\tilde\sigma_1,\ldots,\tilde\sigma_k$.
 In our example the choice is greatly simplified since we consider two variables, i.e. $q=2$. In that case
we can assign assign a uniform prior, $\phi_k\sim\mathcal{U}(-1,1)$,  for the correlation coefficient $\phi_k$ that are supposed identically and independent distributed.
	


For sampling
from the posterior distribution we use a hybrid MCMC algorithm known as Metropolis-within-Gibbs algorithm \citep[][Chapter 10]{Robert2004}.
As we show in the Supplementary material the conjugacy of some priors leads to  updates with
simple, established methods for drawing from the full
conditional distribution.
In other cases, we  resort to Metropolis-Hastings
to draw from some of the full conditional distributions.




==> Bivariate Quantile Regression Clustering/results.tex <==
\section{Clustering sites in the Gulf of Gabes}\label{sec5}

In this section we present the clustering results for the bivariate variables Chl-a concentration and the KD-490 levels, previously presented in Section \ref{sec2}.  
As reported in Figure \ref{fig:2}, we can observe a strong and time-varying seasonal pattern, with the presence of a peak at the beginning of each year. For this reason
 we choose to model such monthly seasonality using sine and cosine functions \citep{eilers2008modulation}.
 More precisely we suppose that for each variable $y$ the quantile regression function is a function of the time $t$, such that 
 \begin{equation*}%\label{eq5.bis}
Q_p(y|t)=g_1(t)+ g_2(t) \cos(\pi/6t)+ g_3(t) \sin(\pi/6t)
 \end{equation*}
 where   a possible overall trend is represented by a smooth function $g_1(t)$, while $g_2(t)$ and $g_3(t)$ are smooth functions  that modulate the local amplitudes of the cosine and sine waves. 

In order to have a good grade of flexibility, the three  functions $g_1(t)$, $g_2(t)$, and $g_3(t)$ take the form of a regression on a cubic B-spline basis, $
g_j(t)= \sum_{l=1}^{m_j} \beta_{jl} b_l(t)
$
with  equally spaced knots over the time interval $[1,108]$.
It is easy to see that the resulting  model for the quantile function
 \begin{equation*}%\label{eq5.bis}
	Q_p(y|t)=\sum_{l=1}^{m_1} \beta_{1l} b_l(t)+ \sum_{l=1}^{m_2} \beta_{2l}[b_l(t)\cos(\pi/6t)]+ \sum_{l=1}^{m_3} \beta_{3l}[b_l(t)\sin(\pi/6t)]
\end{equation*}
can be written as a linear combination of covariates  that fits with \eqref{eq:ald}.

We carry out a preliminary data analysis in order to get the degree of smoothing and the number of clusters.
This data  analysis has been performed on the time series  of Chl-a concentration since this variable displayed more heterogeneity in space and time.


To find the  grade of smoothing and obtain a value for $m_1$, $m_2$, and $m_3$, we follow the strategy outlined in Section \ref{sec4} and we minimize the overall value $AIC(m)$, with  $m=m_1+m_2+m_3$  by means of a median (i.e. $p=0.5$) regression.  
The solution with $m_1=4$ for the  trend (with the inclusion of a internal intercept) and $m_2=m_3=3$ for the cyclical components minimized the overall $AIC(m)$ and it was chosen  in the model.
Having fixed the number of covariates and still fixing $p=0.5$ we  identify the number of clusters, $K=5$ by minimizing  the  conditional version named $DIC_8$ \citep{celeux2006deviance} of
Deviance Information Criteria \citep{spiegelhalter2002bayesian}.

Then we fit a bivariate model assuming that the two time series have a constant correlation coefficient across the clusters, i.e. $\phi=\phi_k$.
Moreover a word of caution is in order of the estimate of the parameter $\gamma$ in \eqref{eq:downton}. Our experience with this dataset indicates that the the data provide very little information on the parameter. For this reason we set the value $\gamma=0.5$,
giving the parameter $\phi$ the task of modulating the dependence 
between the two time series.

 We estimate the model for a range of different quantile combinations namely for different values of $(p_{1},p_{2})$. Particularly we consider the combination of quantiles given by the pairs $ (0.5,0.5) $, $ (0.9,0.5) $, and $ (0.9,0.9) $ for Chl-a concentration and KD-490, respectively.

The results were obtained after 2500 Monte Carlo iterations using a burn-in of 200. The final membership ${c}_i$ and the regression coefficients $\beta_{jl}$ were estimated by means of the mode and mean of a-posteriori distribution, respectively. In Figure \ref{spatial} we present the spatial distribution of the clustering results for each combination quantiles.



Across all the fitted quantile combinations, we observe that those regions around the islands (Kerkennah, Kneiss and Jerba) are clustered as having the highest average values of both Chl-a and KD-490 concentration which decreases as one moves towards the deep sea. These results are consistent with the results obtained from the univariate case as well as the findings of \cite{Katlane2012} who notes that, from multi-temporal turbidity maps produced from Moderate Resolution Imaging Spectrometer (MODIS) for $ 2009 $, areas around the islands (Kerkenah, Kneiss and Jerba) and at the industrial port of Gannouch, were characterized by high turbidity variation, concentration of total suspended matter and Chl-a concentration.

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{spatial_results.png}
	\caption{Spatial clustering results for Chl-a concentration and KD-490 index at quantile combination (a) $ (0.5,0.5)$, (b) $ (0.9,0.5)$, and (c) $ (0.9,0.9). $\label{spatial} }
\end{figure}

However, given the different meaning of Chl-a concentration and KD-490 levels at each quantile level, the spatial distribution between the three classifications appears different in particular looking to the northeastern area and to coastal zone. In fact the classification with (0.5,0.5) identifies a series of clusters which describe not only the most polluted area (Cluster $4$ and $5$), but also the coastal area (Cluster $3$) and the zone inside the Gulf (Cluster $2$). Otherwise, the classification in (0.9,0.5) and  (0.9,0.9) reported a wide cluster $1$ which covers a zone starting from the offshore waters to the coastal area, with the exception of the islands and the Sfax industrial area in the north-east.  In fact, as reported in Figure \ref{boxplots}, the classification performed with the quantile combination (0.5, 0.5) reported an increasing trend of both Chl-a concentration and KD-490 levels. The clustering performed with a quantile combination of 0.9 for Chl-a and 0.5 for KD-490 appears different with respect to the combination $(0.5,0.5)$ both in terms of group size and the median values across clusters: cluster $1$ embraces the 88.6\% of the sites and the Chl-a values of the cluster $2$ and $3$ overlapped as well as those of the cluster $4$ and $5$; low KD-490 levels are restricted to the cluster $1$ while the cluster $4$ reports the highest one. In the classification with the quantile combination $(0.9,0.9)$, the number of sites which belongs to cluster $1$ increases (94.4\%) while cluster $3$ and $4$ are represented by only 3 and 8 sites, respectively. The Chl-a values in the cluster $1$ are low and well separated by the cluster $2$ and $5$; the KD-490 levels of the cluster $2$ and $5$ are similar. The meaning of the classification with the quantile combination $(0.9,0.9)$ is similar to those of the previous classification $(0.9, 0.5)$, but with a greater spatial continuity among the cluster membership.
For both the  classifications with the quantile combination $(0.9, 0.9)$ and $(0.9,0.5)$, especially the last, some clusters are represented by a low number of sites indicating that a lower number of cluster may be more appropriate.


\begin{figure}[h!]
	\centering
	\includegraphics[width=1\textwidth]{boxplots.png}\\
	\caption{Distribution of Chl-a concentration and KD-490 index by Cluster fo each quantile combination (a) $ (0.5,0.5) $, (b) $ (0.9,0.5)$ and  (c) $ (0.9,0.9). $\label{boxplots} }
\end{figure}

In Figure \ref{timeseries} the temporal pattern for each recovered cluster is reported by plotting the estimated quantile functions  of Chl-a concentration and KD-490 for each considered combination of quantiles. For all cluster a seasonal pattern is evident. Cluster labels and colors are the same as those in Figure \ref{spatial}. %and they are ordered by average $\hat{g(t)}$ of the Chl-a value. 
The classification with the quantile combination $(0.5,0.5)$ is guided by different average levels in Chl-a concentration with the last cluster looking different from the others; the clustering on KD-490 identifies five clusters with different average values and denotes an increasing trend for the Clusters $4$ and $5$ at the beginning of the time window followed by an increasing oscillation.
Considering the clustering results obtained by the quantile combination $(0.9-0.5)$, the temporal trend appears different with respect to the previous classification: Clusters from $2$ to $5$ reported an increasing trend and a stabilization after 2007 for both Chl-a and KD490 indicators; the seasonal component appears more evident in the quantile 0.5 of KD-490 levels than in the quantile 0.9 of the Chl-a concentration; Chl-a concentration of Clusters $4$ and $5$ appears to be similar in average, but the oscillation in the Cluster $5$ is smoothed. For the KD-490, Cluster $4$ reports the highest level, followed by Cluster $5$ and then by $3$ and $2$, very close to each other. The Cluster $1$ showed the lowest values and a wide distance from the other groups for both the indicators. The clustering of the quantile combination $(0.9-0.9)$ shows: an increasing trend and a stabilization after 2007 only for the Chl-a concentration for the Clusters $2$, $3$, and $5$; Clusters from $2$ to $5$ report a similar behaviour; with the exception of the first cluster, KD-490 levels are similar among the identified pair of Clusters $5$ and $2$, and $3$ and $4$, with a decreasing amplitude in the cluster $4$. For both the indicators Cluster $1$ reports values far from the other groups.

\newpage
\begin{figure}[h!]
	\centering
%	\text{(a)}
	\includegraphics[height=0.3\textheight]{time_series0505.png}\\
%	\text{(b)}
	\includegraphics[height=0.3\textheight]{time_series0905.png}\\
%	\text{(c)}
	\includegraphics[height=0.3\textheight]{time_series0909.png}\\
	\caption{Average quantiles for Chl-a concentration and KD-490 index at several combinations of percentages $(p_1,p_2)$.  $ (0.5,0.5)  $ (top),  $ (0.9,0.5)$ (middle), and   $ (0.9,0.9) $ (bottom). \label{timeseries} }
\end{figure}


==> Bivariate Quantile Regression Clustering/revision/data.tex <==
\section{Chl-a and KD-490 levels in the Gulf of Gabes}\label{sec2}
The Gulf of Gabes is a Mediterranean zone with important biological resources and rich coastal, marine and freshwater ecosystems. In the last decades the Gulf of Gabes reported several environmental problems mainly due to the presence of human activities associated with over-fishing and seabed trawling while the presence of chemical factories in the Sfax site resulting on a wide wastewater pollution \citep{Aloulou:2012,Rabaoui:2013,Zaghden:2014,Fourati:2018}.
The results had led  to  several issues as the local appearance of red tides \citep{hamza:1994} as well as the changes or decline of the distribution of some marine species \citep{el:2016,el:2018}.

The European Community indicates  the diffuse Chlorophyll type-a (Chl-a) concentrations as a trophic status indicator of the sea-water. High Chl-a levels may lead to hypoxic or anoxic events.  KD-490 indicates how the solar light can penetrate to deeper water and can be used to evaluate the potential disturbance to the water ecosystem.

In this work, we considered two datasets comprising the Chl-a concentrations and the KD-490 levels made available by ACRI (\texttt{hermes.acri.fr}) in the framework of the GlobColour Project (\texttt{www.globcolour.info}).
The datasets were formed by monthly values of Chl-a concentrations and KD-490 levels in the Gulf of Gabes from January, 2003 to December, 2011 for a total of $108$ time-points. Data were obtained by calibrating Ocean Colour data provided by different satellite missions, such as MERIS, SeaWiFS and MODIS. For each month, gridded data with 1.8-km resolution are available and  a  grid of $4,033$ points  covers the entire Gulf of Gabes.
\begin{figure}
	\centering
	\begin{tabular}{c}
%		\includegraphics[width=0.9\linewidth]{revision/fig2a.pdf}  \\
%		\includegraphics[width=0.9\linewidth]{revision/fig2b.pdf} \\
%		%(a) & (b)
\includegraphics[width=0.95\linewidth]{revision/Figure1.pdf} 
	\end{tabular}
	\caption{\textcolor{black}{Temporal profile for the quantiles (0.05, 0.25, 0.50, 0.75, and 0.95). For each time we calculated the empirical quantiles over the 4033 time-series.}}\label{fig:2plus}
\end{figure}
\textcolor{black}{As reported in Figure \ref{fig:2plus}, both Chl-a concentrations and KD-490 levels exhibit a seasonal cyclical pattern, more evident in the case of chlorophyll, with the presence of a peak during the spring period. While the KD-490 is related to the sea water turbidity more or less correlated to environmental factors (heavy rain, wind direction, etc\dots), the Chl-a index reflects the seasonal bloom in vegetation, directly connected to the seasonal variation of the sunlight window and the sea water temperature.}



%%%decribe the tow figures 
In Figure \ref{fig:1} we report the average levels of Chl-a concentration and KD-490 index for all the sites \textcolor{black}{over the spatial domain}.
% describe the temporal trend of the selected sites.
%%%%%%%%%%%%%%%

\begin{figure}
	\centering
	\begin{tabular}{cc}
%		\includegraphics[width=0.5\linewidth]{revision/meanChla_trim.png}  &
%		\includegraphics[width=0.5\linewidth]{revision/meanKD490_trim.png} \\
	\includegraphics[width=0.95\linewidth]{revision/Figure2.png}
		%(a) & (b)
	\end{tabular}
	\caption{Observed grid-points (4033 sites) in the Gulf of Gabes for the average Chl-a (left) and KD-490 (right) and two example sites reported in Figure \ref{fig:2}. \textcolor{black}{White color near the coastal area corresponds to sites with no values due to shallow waters.}}\label{fig:1}
\end{figure}
The highest average levels of Chl-a and KD-490 were reported near the coastal area, in the north-eastern zone (Sfax) and in the southern part (Djerba) of the Gulf. The spatial distribution of the average values between Chl-a and KD-490 appears to have a similar spatial and temporal behaviour, but not everywhere. In fact as shown in Figure \ref{fig:2} the example site 1 exhibits a strong seasonal pattern both in the Chl-a and KD-490 indicators, with a strong correlation between the two time series (Pearson $\rho$: 66.1\%); in the second example site 2 there is a clear difference between the trend of the Chl-a concentration with respect to the KD-490 one as attested by a weak correlation (Pearson $\rho$: 30.7\%).

\begin{figure}
	\centering
	\begin{tabular}{c}
%		\includegraphics[width=0.5\textwidth]{revision/example1.png}  &
%		\includegraphics[width=0.5\textwidth]{revision/example2.png} \\
\includegraphics[width=0.95\textwidth]{revision/Figure3.png}\\
\hspace{-1cm}(1) Lat: 10.88; Long: 33.99 \hspace{2.1cm} (2) Lat: 11.08; Long: 34.86\\
	\end{tabular}
	\caption{Temporal trend of Chl-a and Kd-490 in the two selected example sites.}\label{fig:2}
\end{figure}

The dataset is affected by outliers due to measurement errors  (Chl-a concentration lower than 0.05 $mg/m^{-3}$: 1.0\%; KD-490 levels lower than 0.05 $m^{-1}$: 2.8\%) and by a  different amount of missing observations
% please verify how many observations are missing
(Chl-a: 19.1\%; KD-490: 1.8\%). 
The presented dataset presents several features which makes the clustering task challenging: a strong seasonality and a high variability,  the presence of outliers and a non bell-shaped distribution. The proposed classification may help to assess the trophic status of this area combining the information provided by different temporal Chl-a and KD-490 levels.

==> Bivariate Quantile Regression Clustering/revision/discussion.tex <==
\section{Discussion}\label{sec6}
In this paper we have proposed a new model-based clustering technique,  that is capable of handling asymmetric clusters with the presence of outliers as well as considering different quantile levels of the observed data. Our clustering strategy is based on the finite mixture model theory where each component of the mixture of AL distributions, which constitutes  the density of bivariate random variables which are potentially correlated, is assumed to represent a cluster with the skewness parameter of AL distribution being used to directly model the quantiles of interest. Therefore our proposed technique adds to the richness of the recent burgeoning of non-Gaussian approaches to model-based clustering.

\textcolor{black}{As the AL distribution provides a direct link between the maximum likelihood theory and minimization of a quantile regression check loss function \citep[see][]{koenker1999goodness,yu2001bayesian}, we estimate the cluster-specific  parameters, which are the parameters of the mixing AL distribution, through a Bayesian %quantile regression 
approach.} 
%Following from \cite{Waldmann2015} we implement our bivariate clustering model
%that is based on Bayesian bivariate quantile regression. We note that due to the dependence on the constructed likelihood for the bivariate random variables there are no closed-form available conditional distributions for the model parameters. Therefore we introduce MH steps to estimate the parameters through MCMC. 

In our simulation experiment we considered three clusters two of which are not distinctively different from each other. However, an evaluation of the power of our proposed algorithm in reconstructing the three groups indicates a good performance with respect to the other competitive methods. We have applied the procedure to time series observed from GlobColour data related to Chlorophyll type-a concentrations and KD-490 levels in order to identify homogeneous areas in the Gulf of Gabes with respect to the temporal behavior of these water indicators \textcolor{black}{by means of a seasonal modulation model}. We defined clusters that are similar by different combination of quantiles of the two indicators. It is important to note that as different choice of quantiles implies changes in the clustering, this method may be particularly suitable for defining areas at different risk when considering two indicators at different quantile levels. More particularly, important features are of absolute interest in environmental sciences and ecology \citep{schmidt2012estimating}.
\textcolor{black}{In addition, the use of a model matrix based on a seasonal modulation model is evoked by the periodic behaviour of time series in our environmental application; however other flexible specifications can also be adopted.}

We note that both Chl-a concentrations and KD-490 levels are affected by several spatially varying factors. \textcolor{black}{Potential consequences of non incorporating in the model information related to the spatial domain may result from misclassification to  lower predictive ability; the spatial dependence can be particularly helpful in presence of high percentage of missing data. In this case potential future development of the modelling approach   can be the incorporation of  spatial dependence among the probabilities of membership as in   \cite{jiang2012clustering} or  \citet{Gaetan:2017}}.
Another possible extension is to perform clustering at multiple quantiles instead of fixing the levels of quantiles. However, caution has to be taken in this case to avoid the issue of crossing quantiles.


==> Bivariate Quantile Regression Clustering/revision/methods.tex <==
\section{Statistical modelling and inference}\label{sec3}
 \subsection{Multivariate quantile regression and asymmetric Laplace distribution}
We start by considering the  univariate case.
 Let $ Q_{p}(y|x) $, for $ 0<p<1 $, be the $p$-th quantile regression function of the univariate continuous random variable $ y $ given $ x$, a vector of  covariates.
 We suppose that $ Q_{p}(y|x)=x'\beta $, where $ \beta $ is a vector of unknown parameters to be estimated. Then a quantile regression model can be defined as $y=x'\beta+e$
where $ e$ is an error term  with  density function $f(\cdot;p) $ and  the $ p $-th quantile equal to zero, i.e. $ \int_{-\infty}^{0}f(e;p)de=p$.
Owing to the data $(y_t,x_t')$, $t=1,\ldots, T$, the  estimate of $\beta$ is classically \citep{koenker1978regression} obtained by minimizing 
\begin{eqnarray}\label{eq2}
	\hat{\beta}=\underset{\beta}{\text{argmin}}\sum_{t=1}^{T}\rho_{p}(y_{t}-x_{t}'\beta),
\end{eqnarray}
where $ \rho_{p}(\cdot) $ is the check loss function, i.e. $ \rho_{p}(z)=z(p-I(z<0)) $.

\citet{koenker1999goodness} showed that there is a direct relationship between minimizing (\ref{eq2}) and the maximum likelihood theory using independent variables $y_t$ with  Asymmetric Laplace   (AL) density
\begin{equation}
	f(e;p)=\frac{p(1-p)}{\sigma}\exp\left\{-\rho_{p}\left(\frac{e}{\sigma}\right)\right\},\label{eq3}
\end{equation}
where $ \sigma>0 $  is an additional   scale parameter.

In the following we will exploit the representation of $y$ with density \eqref{eq3} as a location scale mixture of Gaussian random variable  \citep{Kotz2001}, namely
\begin{eqnarray}
	y=x'\beta+\theta \sigma w+\omega \sigma\sqrt{ w}\,\nu \label{eq5}
\end{eqnarray}
where $ \nu\sim \mathcal{N}(0,1) $, and $ w $ is a exponential random variable with  $E(w)=1$. Here $\nu $ and $ w $ are mutually independent and
$\theta=(1-2p)/\{p(1-p)\}$ and $\omega^{2}=2/\{p(1-p)\}$.


The literature has focused on univariate response variable with only a few studies considering extension to multivariate case \citep{Benoit2012,Benoit2013,Waldmann2015,Petrella2019a}.


In particular \cite{Petrella2019a} considered a multivariate  asymmetric Laplace distribution \citep{Kotz2001} to specify a quantile regression model for the random vector
$\tilde{y}=(y_1,\ldots,y_q)'$ in the mixture representation
\begin{equation}
	\tilde{y}=X'\tilde{\beta}+ D\Theta {w} +\sqrt{w}D\Sigma^{1/2}\tilde{\nu} \label{eq3.20}
\end{equation}

Here  $\tilde{\nu}$ denotes a $q$-dimension standard Gaussian vector and $w$ is a exponential random variable with unit mean.
The matrix $X$ is a $q\times L$  regressor matrix and $\tilde\beta$ is a $L$-dimensional unknown vector. The other parameters of the model are contained in  $D = \operatorname{diag}(\tilde\sigma)$, with $\tilde{\sigma}=(\sigma_1,\ldots,\sigma_q)'$,  $\sigma_j>0$, $j=1,\ldots,q$  and $\Theta= \operatorname{diag}(\theta_1,\ldots,
\theta_q)'$ with $\theta_j = (1 - 2p_j)/[p_j (1 - p_j]$. 

Moreover the matrix $\Sigma=\Omega R(\tilde\phi)\Omega$ is a $q \times q$ positive definite matrix   with $R(\tilde\phi)$ being a correlation matrix, that depends on a vector of parameters $\tilde\phi$, and $\Omega= \operatorname{diag}(\omega_1^2,\ldots,\omega_q^2)$,
with entry $\omega_{j}^{2}={2}/[p_{j}(1-p_{j})]$. Note that using this formulation the component $y_j$ will  always be mutually dependent, even though $R(\phi)$ is an identity matrix.

In this paper we  consider a slight different approach with respect to  \eqref{eq3.20}.
We use the same idea as in \cite{Waldmann2015} and we set

\begin{equation}\label{eq:ald}
	\tilde{y}=X'\beta+ D\Theta \tilde{w} +{W}^{1/2}D\Sigma^{1/2}\tilde{\nu} 
\end{equation}
with $\tilde{w}= ({w}_1,\ldots,w_q)'$ and ${W}= \operatorname{diag}({w}_1,\ldots,{w}_q)$
allowing a different  exponential random variable with unit mean $ w_j$ for each component.


With this variation   model \eqref{eq:ald} does not define a proper multivariate asymmetric Laplace distribution as in \citet{Kotz2001}. However the model becomes more flexible and can cover the case of mutually independent components.
Now the challenge  lies in finding a multivariate density
for $\tilde{w}$, $	e(\tilde{w};\gamma)$, with marginal exponential distributions for the $w_j$ in order to guarantee that the marginal distributions for the response variables are still asymmetric Laplace. Here the parameter $\gamma$ is a generic dependence parameter.
%Therefore the multivariate density function of \eqref{eq:ald}
%\begin{eqnarray}
%	\textrm{ald}(\tilde{y}|\tilde{x},\beta,D,R(\phi),\gamma) 
%	&=&\int_{(0,\infty)^q} (2\pi)^{-q/2}|W^{{1}/{2}}\varSigma W^{{1}/{2}}|^{-{1}/{2}}\times \nonumber\\
%	&& \exp\left\{-\frac{1}{2}(\tilde{y}-X'\beta- D\Theta \tilde{w})'W^{-{1}/{2}}\varSigma^{-1}W^{-{1}/{2}}(
%	\tilde{y}-X'\beta- D\Theta \tilde{w})\right\}\times\nonumber\\
%	&& f(\tilde{w};\gamma)d\tilde{w}
%\end{eqnarray}

Several multivariate exponential distributions   have been proposed in the literature \citep[Ch. 47]{kotz:balakrishnan:johnson}.
\cite{Waldmann2015} adopt the simplest specification that the exponential variables are independent, i.e. $\gamma=0$.

In view of the bivariate real data example in this paper we exemplify our construction by using the bivariate density proposed by \cite{Downton1970}, namely
\begin{equation}\label{eq:downton}
	e(\tilde{w};\gamma)= \frac{1}{(1-\gamma)}\exp \left\{-\frac{1}{1-\gamma}\left(w_{1}+w_{2}\right)\right\}
I_{0}\left(\frac{2}{1-\gamma}\sqrt{\gamma w_{1}w_{2}}\right)
\end{equation}
where $ 0\le\gamma < 1 $
and $I_{0}(a)=\sum_{k=1}^{\infty}\frac{a^{2k}}{4^{k}(k!)^{2}}$ is the modified Bessel function of the first kind of order zero.
The value $\gamma$ represents the 
Pearson's product-moment correlation and $ \gamma=0 $ implies independence between the $w_1$ and $w_2$.
Coupling \eqref{eq:ald} with the density \eqref{eq:downton} we obtain a  flexible specification of a bivariate quantile regression model that covers the case of independence between  the components when $R(\phi)$ is an identity matrix and $\gamma=0$.




\subsection{Model-based clustering}\label{subsec:mixmod}
Suppose that we observe  data over $n$ statistical units and, for simplicity,  the same number $q\times T$  of values $y_{ijt}$,  $j=1,\ldots, q$, $t=1,\ldots,T$, for each statistical unit $i$, $i=1,\ldots,n$.
We collect the observations for each unit into the vector $\boldsymbol{y}_i = (\tilde{y}_{i1}',\ldots, \tilde{y}_{iT}')'$, with
$\tilde{y}_{it} = (y_{i1t},y_{i2t},\ldots y_{iqt})'$, $t=1,\ldots,T$.
The vectors  $\boldsymbol{y}_i$ are supposed to be independent.
The whole dataset will be denoted by $\mathcal{Y}=(\boldsymbol{y}_1,\ldots,\boldsymbol{y}_n)$.

Our statistical  problem is to cluster the $n$ statistical units, i.e. the sites,  into the clusters $\{1,\ldots,K\}$, $K\ll n$.
We follow a  mixture-model  approach \citep{mclachlan:peel:2000}  to clustering  according to which the cluster membership of the $i$th unit is represented by a latent random variable  ${c}_i \in \{1,\ldots,K\} $ , where $c_{i} = k$ indicates if the $i$-th units belongs to the cluster $k$. 

The memberships ${c}_i$, $i=1,\ldots,n$ are supposed independent and identically distributed  variables with 
$\Pr(c_{i} = k)=\alpha_k$, $ 0<\alpha_{k}<1 $, for all $k=1,\ldots,K$ and $ \sum_{k=1}^{K}\alpha_{k}=1 $.



Given the cluster membership,  $c_{i}$,  observations for the $i$-th unit are generated by the mixture model specified hierarchically, namely 

\noindent\textbf{the observation level}
\begin{equation}\label{eq:model}
		\tilde{y}_{it}|c_i,\tilde{w}_{it}\sim\mathcal{N}_q(X_{t}'\tilde\beta_{c_i}+ D_{c_i}\Theta \tilde{w}_{it},{W}_{it}D_{c_i}\Sigma_{c_i}D_{c_i}{W}_{it}), \qquad i=1,\ldots,n,\quad t=1,\ldots,T 
\end{equation}
		conditionally independent distributed, with $\Sigma_{c_i}=\Omega R(\phi_{c_i})\Omega$;

\noindent \textbf{the latent process level}
\begin{equation}
		\tilde{w}_{it}|c_i\sim e(w,\gamma_{c_i}), \quad i=1,\ldots,n,\quad t=1,\ldots,T
\end{equation}
		conditionally independent distributed
\begin{equation}
		c_i \sim \operatorname{Multinomial}(1,{\alpha}), \quad i=1,\ldots,n
\end{equation}
independent distributed.  
\textcolor{black}{However, in presence of statistical units over a spatial domain, the incorporation of the spatial dependence in the model can be a feature that needs to be considered. Since the aim of our main application (see Section \ref{sec5}) was to discover sites at different environmental pressure, the incorporation of spatial dependence in the MCMC chain can eventually mask the classification by a common smoothing effect. Depending on the type of spatial domain and the analysed data,  this dependence can be incorporated, for example, by considering a Markov random field as, for example, in \citep{Gaetan:2017,jiang2012clustering} that takes into account the membership of the nearest neighbors.}

\subsection{Bayesian inference}\label{subsec:bayinf}
We adopt a Bayesian approach to make inference on the model parameters.
The inference is facilitated by the fact that the mixture model is  specified hierarchically. Moreover
the conjugacy of some priors leads to  updates with
simple and established methods for drawing from the full
conditional distribution.
%Moreover it is possible to get the posterior probability of membership of a single vector, $\Pr(c_i=\cdot|\mathcal{Y})$.


\noindent \textbf{Prior distributions}

A common choice for the prior distribution of $\alpha$ is $ {\alpha}\sim \mathcal{D}(a_{1},...,a_{K}) $, where $\mathcal{D}$ is the Dirichlet distribution with parameters $a_1, \ldots, a_K > 0$;  % which is a conjugate prior for the mixing proportions

The choice $ \tilde\beta_{k} \sim \mathcal{N}(b_k,P_k),\, k=1,\ldots,K$, identically and independent distributed is still common and simplifies the simulation. Setting $ b_k=0 $ and $ P_k=a\,I $, for $ a \gg 0 $, leads to an improper prior.
		
		 Specification of the  prior distributions for
		$\tilde\sigma_1,\ldots,\tilde\sigma_k$ and $\tilde\phi_1,\ldots,\tilde\phi_k$  is complicated  by the complex requirement that the matrices $D_k\Omega R(\phi_{k})\Omega D_k$ are  non-negative definite matrices.
We follow \citet{barnard:mcculloch:meng:2000} and   work  by specifying prior for variances  and correlation matrices.
For the variances we put the priors $ \sigma^2_{kj} \sim \mathrm{IG}(s_{k},d_{k}),\quad k=1,\ldots,K,\quad j=1,\ldots,q$,  identically and independent distributed,
	where $IG$ is  the inverse gamma distribution,
	with the shape $ s_{k}$  and $ d_{k}$ scale parameters.
	\citet{barnard:mcculloch:meng:2000} discussed the relative merits of choosing a prior for $\tilde\phi_1,\ldots,\tilde\phi_k$ independent from $\tilde\sigma_1,\ldots,\tilde\sigma_k$.
 In our example the choice is greatly simplified since we consider two variables, i.e. $q=2$. In that case
we can assign assign a uniform prior, $\phi_k\sim\mathcal{U}(-1,1)$,  for the correlation coefficient $\phi_k$ that are supposed identically and independent distributed.
	


For sampling
from the posterior distribution we use a hybrid MCMC algorithm known as Metropolis-within-Gibbs algorithm \citep[][Chapter 10]{Robert2004}.
As we show in the Supplementary material the conjugacy of some priors leads to  updates with
simple, established methods for drawing from the full
conditional distribution.
In other cases, we  resort to Metropolis-Hastings
to draw from some of the full conditional distributions.




==> Bivariate Quantile Regression Clustering/revision/results.tex <==
\section{Clustering sites in the Gulf of Gabes}\label{sec5}

In this section we present the clustering results for the bivariate variables Chl-a concentration and the KD-490 levels, previously presented in Section \ref{sec2}.  
As reported in Figure \ref{fig:2} and \ref{fig:2plus}, we can observe a strong and time-varying seasonal pattern, with the presence of a peak at the beginning of each year. For this reason
 we choose to model such monthly seasonality using sine and cosine functions \citep{eilers2008modulation}.
 More precisely we suppose that for each variable $y$ the quantile regression function is a function of the time $t$, such that 
 \begin{equation*}%\label{eq5.bis}
Q_p(y|t)=g_1(t)+ g_2(t) \cos(\pi/6t)+ g_3(t) \sin(\pi/6t)
 \end{equation*}
 where   a possible overall trend is represented by a smooth function $g_1(t)$, while $g_2(t)$ and $g_3(t)$ are smooth functions  that modulate the local amplitudes of the cosine and sine waves. 

In order to have a good grade of flexibility, the three functions $g_1(t)$, $g_2(t)$, and $g_3(t)$ take the form of a regression on a cubic B-spline basis, $
g_j(t)= \sum_{l=1}^{m_j} \beta_{jl} b_l(t)
$
with  equally spaced knots over the time interval $[1,108]$.
It is easy to see that the resulting  model for the quantile function
 \begin{equation*}%\label{eq5.bis}
	Q_p(y|t)=\sum_{l=1}^{m_1} \beta_{1l} b_l(t)+ \sum_{l=1}^{m_2} \beta_{2l}[b_l(t)\cos(\pi/6t)]+ \sum_{l=1}^{m_3} \beta_{3l}[b_l(t)\sin(\pi/6t)]
\end{equation*}
can be written as a linear combination of covariates  that fits with \eqref{eq:ald}.

We carry out a preliminary data analysis in order to get the degree of smoothing and the number of clusters.
This data  analysis has been performed on the time series  of Chl-a concentration since this variable displayed more heterogeneity in space and time.


To find the  grade of smoothing and obtain a value for $m_1$, $m_2$, and $m_3$, we follow the strategy outlined in Section \ref{sec4} and we minimize the overall value $AIC(m)$, with  $m=m_1+m_2+m_3$  by means of a median (i.e. $p=0.5$) regression \textcolor{black}{and considering a number of basis for each component from 3 to 6.}
The solution with $m_1=4$ for the  trend (with the inclusion of a internal intercept) and $m_2=m_3=3$ for the cyclical components minimized the overall $AIC(m)$ and it was chosen in the following models.


\textcolor{black}{For a fixed number  of clusters $K$, we fit a bivariate model assuming that the two time series have a constant correlation coefficient across the clusters, i.e. $\phi=\phi_k$.
Moreover a word of caution is in order of the estimate of the parameter $\gamma$ in \eqref{eq:downton}. Our experience with this dataset indicates that the data provide very little information on the parameter. For this reason we set the value $\gamma=0.5$, giving the parameter $\phi$ the task of modulating the dependence between the two time series.
}

\textcolor{black}{The results were obtained after 2500 Monte Carlo iterations using a burn-in of 300. The final membership ${c}_i$ and the regression coefficients $\beta_{jl}$ were estimated by means of the mode and mean of a-posteriori distribution, respectively.}


\textcolor{black}{We identify $K$ minimizing an adapted  version of the Deviance Information Criterion ($DIC$) \citep{spiegelhalter2002bayesian} following \citet{celeux2006deviance}. More precisely starting from the formulation   named $DIC_2$ in that paper
}
$$
DIC_{2}(\mathbf{y},\mathbf{\psi})= -4\mathbb{E}_{\psi,\mathcal{C}}[\text{log}f(\mathbf{y}|,\psi)|\mathbf{y}]+2\text{log}f(\mathbf{y},\tilde{\psi}(\mathbf{y})) \label{eq2.27}
$$
\textcolor{black}{
where $\mathbf{\psi} =(\mathbb{\beta},\sigma)'$ and $\tilde{\psi}(\mathbf{y})$ is the  maximum a posteriori (MAP) estimates of ${\psi}$.   \citet{celeux2006deviance}  approximates $ DIC_{2} $  by using the MCMC runs 
}
%\begin{eqnarray}
%DIC (\mathbf{Y},\mathcal{C},\bold{\psi})&\approx& %-\frac{4}{m}\sum_{j=1}^{m}\sum_{i=1}^{n}\sum_{k=1}^{K}\alpha_{ik}(\mathbf{y}_{i},\psi^{(j)})\text{log}f(\mat%hbf{y}_{i}|\psi_{k}^{(j)})\nonumber\\
%&& + 2\sum_{i=1}^{n}\sum_{k=1}^{K}\alpha_{ik}(\mathbf{y}_{i},\bar{\psi})\text{log}\left(f(\mathbf{y}_{i}|\ba%r{\psi}_{k})\right) \label{eq2.29}
%\end{eqnarray}

\begin{eqnarray}
CDIC(\mathbf{y})&=& -\frac{4}{m}\sum_{l=1}^{m}\sum_{i=1}^{n}\log\left\{\sum_{k=1}^{K}
\alpha_{k}^{(l)}
 f(\mathbf{y}_{i}|\psi_k^{(l)})\right\}\nonumber\\
&& +\quad 2\sum_{i=1}^{n}\log\left\{\frac{1}{m}\sum_{l=1}^m \sum_{k=1}^{K}\alpha_{k}^{(l)} f(\mathbf{y}_{i}|\psi_k^{(l)})\right\}\label{eq:dic}
\end{eqnarray}
\textcolor{black}{where $ \psi_k^{(m)} $ and $ \alpha_{k}^{(l)}$ are the results of the $l$-th MCMC iteration.}

\textcolor{black}{However, Formula \ref{eq:dic} entails the evaluation of  the bivariate density function 
$f(y_{i1t}, y_{i2t};\psi_k)$ that arises from equation \eqref{eq:ald} by integrating out the random variable $\tilde{w}$. Since the bivariate  density function cannot be derived in closed form, we proposed a composite version of the DIC index, called Composite-DIC (CDIC), pretending in \eqref{eq:dic} that  $f(y_{i1t}, y_{i2t};\psi_k)=f( y_{i1t};\psi_k)\cdot f(y_{i2t};\psi_k)$ in the same spirit of \cite{varin2005}.}


 We estimate the model for a range of different quantile combinations namely for different values of $(p_{1},p_{2})$. In particular we consider the combination of quantiles given by the pairs $ (0.5,0.5) $, $ (0.9,0.5) $, and $ (0.9,0.9) $ for Chl-a concentration and KD-490, respectively. \textcolor{black}{While the quantile 0.5 can represent a robust estimate of the central tendency of the behaviour of each indicator, the quantile 0.9 is particularly important in ecology to evaluate the temporal trend towards the upper end of the distribution.}



\textcolor{black}{The values of  CDIC for a number of clusters $K$ which varies from 2 to 7 are reported in Table \ref{tab_cdic}. }  

\begin{table}[ht]
\centering
\textcolor{black}{
\begin{tabular}{cccc}
 \hline
%& \multicolumn{3}{c}{$(p_1,p_2)$ combination}\\
 $K$ &    {(0.5,0.5) }& {(0.9,0.5) }&    {(0.9,0.9)}\\
 \hline
7 & 33.1   & 46.1     & 48.4 \\
6 & \textbf{31.2}        & 44.1      & 46.5      \\
5 & 33.1     & 44.0      & 48.2   \\
4 & 35.1       & \textbf{39.8} & 46.9   \\
3 & 32.3  & 44.1     & \textbf{46.4}     \\
2 & 39.5   & 41.0        & 46.6\\       
 \hline
\end{tabular}
}
	\caption{\textcolor{black}{CDIC ($\times 10^5$) values for $K$  at different quantile pairs. The lowest CDIC value is highlighted in bold.} \label{tab_cdic} }
\end{table}
\textcolor{black}{Considering the values reported in Table \ref{tab_cdic} we have chosen a number of clusters equal to K = 6, 4 and 3 for the quantile combination $ (0.5,0.5) $, $ (0.9,0.5) $ and $ (0, 9,0,9) $, respectively. This result suggests  a different number of clusters for each combination indicating a decreasing number to an increasing combination of quantile levels. Especially for the latest model, the proposed criterion suggests a classification based on three clusters.}



In Figure \ref{spatial} we present the spatial distribution of the clustering results for each combination of quantiles.

Across all the fitted quantile combinations, we observe that those regions around the islands (Kerkennah, Kneiss and Jerba) are clustered as having the highest average values of both Chl-a and KD-490 concentration which decreases as one moves towards the deep sea. These results are consistent with the results obtained from the univariate case as well as the findings of \cite{Katlane2012} who notes that, from multi-temporal turbidity maps produced from Moderate Resolution Imaging Spectrometer (MODIS) for $ 2009 $, areas around the islands (Kerkenah, Kneiss and Jerba) and at the industrial port of Gannouch, were characterized by high turbidity variation, concentration of total suspended matter and Chl-a concentration.

\begin{figure}[ht]
  \centering
%\includegraphics[width=0.3\linewidth]{revision/res0505_trim.png}
%\includegraphics[width=0.3\linewidth]{revision/res0905_trim.png}
%\includegraphics[width=0.3\linewidth]{revision/res0909_trim.png}
\includegraphics[width=0.95\linewidth]{revision/Figure4.png}
	\caption{Spatial clustering results for Chl-a concentration and KD-490 index for each quantile combination $(p_1,p_2)$: (a)  $ (0.5,0.5)$ (left), (b) $ (0.9,0.5)$ (middle), and (c) $ (0.9,0.9)$ (right). \label{spatial} }
\end{figure}


\textcolor{black}{However, given the different meanings of Chl-a concentration and KD-490 levels at each quantile level, the spatial distribution between the three classifications appears different in particular looking at the northeastern area and the coastal zone. The classification with the quantile combination ($0.5,0.5$) identifies a series of clusters that grades not only the most polluted area (Cluster $6$) but also the coastal area (Cluster $4$ and $5$). The zone inside the Gulf is classified with the Cluster $3$, while the remaining zone far from the coastal area and islands is covered by the Cluster $1$ and $2$. Otherwise, the classification with ($0.9,0.5$) reported a similar spatial extension concerning the Cluster $1$ and $2$ which include zones starting from the offshore waters to the coastal area, while the coastal zone and the Sfax industrial area in the north-east are entirely covered by the Cluster $4$; the Cluster $3$ defines a transition zone. As reported in Figure \ref{boxplots}, both the classification performed with ($0.5,0.5$) and ($0.9,0.5$) report an increasing trend in the observed values of both Chl-a concentrations and KD-490 levels with the increase of the cluster label. 
The clustering performed with a quantile combination of 0.9 for Chl-a and 0.5 for KD-490 appears different with respect to the combination $(0.5,0.5)$ both in terms of marginal and spatial distribution: in the quantile combination $(0.9,0.5)$ Cluster $4$ embraces an increased percentage of the seawater (24.6\%) and it shows lower values with respect to the previous most impacted area (Cluster $6$) obtained by the classification with quantiles $(0.5,0.5)$; low KD-490 and CHL-a concentrations are restricted for both the classifications ($(0.5,0.5)$ and $(0.9,0.5)$) to the Cluster $1$, $2$ and Cluster $3$. In the classification with $(0.9,0.9)$, the number of sites that belongs to Cluster $1$ increases to 56.3\%, and the relative spatial extension covers all the offshore water area. The Chl-a and  KD-490 values in the Cluster $1$ are low and widely separated from the Cluster $2$ in comparison with the previous classifications. The sites belonging to Cluster $2$ cover in a unique group all the sites previously classified as a transition zone or near the coastal area. The Cluster $3$ identifies four marine areas heavily impacted by high measurements of Chl-a and KD-490: the seawater around Jerba, Sfax, Zarzis, and Sharqi Island. }


\begin{figure}[!ht]
	\centering
%	\includegraphics[width=1\textwidth]{revision/boxplots.png}\\
	\includegraphics[width=1\textwidth]{revision/Figure5.png}\\
	\caption{Distribution of \textcolor{black}{reference quantile} of Chl-a concentration and KD-490 index by Cluster for each quantile combination $(p_1,p_2)$:  $ (0.5,0.5)$ (left), $ (0.9,0.5)$ (middle) and $ (0.9,0.9)$ (right). \label{boxplots} }
\end{figure}

\textcolor{black}{In Figure \ref{timeseries} the temporal pattern for each recovered cluster is reported by plotting the estimated temporal component ($\hat\beta X$) within each identified group of Chl-a concentration and KD-490 level for each considered combination of quantiles. For all clusters a seasonal pattern is evident. Cluster labels and colors are the same as those in Figure \ref{spatial} \textcolor{black}{ and they are ordered by increasing average Chl-a concentration.}
The classification with the quantile combination $(0.5,0.5)$ is guided by different average levels for Chl-a concentration and KD-490 level; however, especially for Chl-a concentration, the first three clusters ($1$, $2$, and $3$) look very close; the presence of a different classification for those groups is explained by a clear separation considering  respective KD-490 levels: posing our attention to KD-490, the curves report different average values, but a similar seasonal component. In addition, the Cluster $6$ reports an increasing trend at the beginning  of the temporal window for both the indicators and a strong cyclical pattern in Chl-a concentration, while the seasonality is less evident for KD-490.}

\begin{figure}[htp]
	\centering
%	\text{(a)}
%	\includegraphics[height=0.3\textheight]{revision/time_series0505.png}\\
%	\text{(b)}
%	\includegraphics[height=0.3\textheight]{revision/time_series0905.png}\\
%	\text{(c)}revision/
%	\includegraphics[height=0.3\textheight]{revision/time_series0909.png}\\
	\includegraphics[width=0.95\linewidth]{revision/Figure6.png}\\
	\caption{\textcolor{black}{Estimated temporal component  for Chl-a concentration and KD-490 index at quantile combinations $(p_1,p_2)$:  $ (0.5,0.5)  $ (top),  $ (0.9,0.5)$ (middle), and   $ (0.9,0.9) $ (bottom). \label{timeseries} }}
\end{figure}


\textcolor{black}{In Figure \ref{boxplots}, considering the two boxplots in the middle related to the clustering results obtained  with the  quantile combination $(0.9-0.5)$, the analysis of the differences between the estimated groups reports as sites belonging to  Cluster $4$ are those with the highest values and a well separated from the other clusters for both the indicators. Otherwise, Cluster $1$, $2$, and $3$ are close together and the difference is mainly due to a different average trend, a greater intra-season amplitude for Cluster $3$, and a late seasonal peak for Cluster $1$, as denoted by the Figure \ref{timeseries}.
In addition, the temporal trend appears to be different from the previous classification: only for KD-490,  Cluster $4$ reports an evident increasing trend, followed by a stabilization and a slight decrease after the year 2008.
Taking into account the clustering results obtained by the quantiles $(0.9-0.9)$,  all clusters are well separated. Cluster $1$ reports the lowest values of limited signal amplitude, while the Cluster $2$ shows a stable and cyclical behaviour, far from other groups. Cluster $3$ exhibits an increasing trend and a stabilization after 2006 only, for Chl-a concentrations, while the KD-490 trend is stable and cyclical.}

==> Bivariate Quantile Regression Clustering/simulations.tex <==
\section{A simulation study}\label{sec4}
\noindent

In this simulation 
study 
we want to exemplify how the mixture model described in subsection \eqref{subsec:bayinf} is able to cluster different bivariate temporal patterns encountered.

We will consider two experiments. A first experiment (Sim A) in which data are generated   from  a symmetric  distributions and a second example (Sim B) in which data come from asymmetric distributions.
In both experiments we assume that $n=300$ statistical units are split into three clusters of size $n_k=100$, $k=1,2,3$.
For each unit we simulate a bivariate vector of length $T=100$
$(y_{1t},y_{2t})'$, $t=1,\ldots,T$ with  time-varying marginal distributions.

Let $z_{jt}$, $j=1,2$, $t=1,\ldots,T$ a standardized Gaussian random variable and $m_{jk}(t) $ a positive function, $k=1,2,3$, $j=1,2$, $t=1,\ldots,T$.
We consider two setting for simulating $(y_{1t},y_{2t})'$, namely


\begin{enumerate}
	\item[Sim A:]  ${y}_{jt}=m_{jk}(t)+\sqrt{m_{jk}(t)/5}\, z_{jt}$;
	\item[Sim B:] ${y}_{jt} = G^{-1}(\Phi(z_{jt});m_{jk}(t)/5,5)$, where
	$\Phi(z)$ is the cumulative distribution function (CDF) of a standardized Gaussian random variable and $G^{-1}(u;a,b)$ is the inverse of the CDF of a Gamma random variable
	with mean $ab$ and variance $ab^2$.	
\end{enumerate}
The $k$ value  in $m_{jk}(t)$ varies between 1 and 3 depending on the cluster membership.
Note that  the marginal distributions were chosen in the way that the means and the marginal variances are equal in the two settings.

The  temporal patterns in each cluster are led by  the function
$
g(t;a,b)=a[2+t/T + \text{exp}\{-(t/T-b)^{2}/0.05\}]
$, that is
\begin{center}
	\begin{tabular}{ccc}
\textbf{Cluster}		&\multicolumn{2}{c}{\textbf{Component}} \\
\hline
		& $j=1$ & $j=2$ \\
		\hline
		$k=1$ & $m_{11}(t) = g(t;1,0.2)$ &$ m_{21}(t) = g(t;1.5,0.8)$\\
		$k=2$ & $m_{12}(t)=g(t;1,0.5)$&$ m_{22}(t)=g(t;1.5,0.2)$\\
		$k=3$& $m_{13}(t)=g(t;1,0.8)$& $ m_{23}(t)=g(t;1.5,0.5)$\\
		\hline
	\end{tabular}
\end{center}


In order to asses the robustness of the procedure in the presence of serial dependence,  we simulate the bivariate time series $(z_{1t},z_{2t})'$ as
 $z_{jt}=v_{jt}+\theta v_{jt-1}$,  $j=1,2$,
%$$
%\begin{array}{ccc}
%z_{1t}&=&\Phi(v_{1t}+\theta v_{1t-1})\\
%z_{2t}&=&\Phi(v_{2t}+\theta v_{2t-1})\\
%\end{array}
%$$
where %$\Phi(\cdot)$ is the cumulative distribution function of a standard Gaussian random variable and 
$(v_{1t},v_{2t})'\sim\mathcal{N}(0,\Sigma_v)$,  is a bivariate white noise, with $\displaystyle \Sigma_v=\frac{1}{1+\theta^2}\left[\begin{array}{cc}
	1& \rho\\
	\rho & 1
\end{array}\right]
$,
  $-1<\rho<1$ and $-1\le\theta\le 1$. By choosing different  values for  $\rho$ and $\theta$, different degrees of mutual and serial dependence are obtained.





In order to capture the temporal component of the  bivariate vector in each cluster, we follow a regression spline approach.  We choose a cubic B-spline basis, $b_1(t),\ldots,b_{m}(t)$, with equally spaced knots over the range of time. For simplicity,
 we assume the same number $m$ of basis functions for both component of $\tilde{y}_t$.  The resulting matrix $X_{t}$ of regressors  in \eqref{eq:model} 
is
$\displaystyle
X_{t}=\left(
\begin{array}{cc}
x_{t}& 0\\
0 & x_{t}\\
\end{array}
\right)'
$
with $x_t=(b_1(t),\ldots,b_{m}(t))'$.

We suggest this simple strategy for a  preliminary selection of the number of basis $m$, namely
\begin{enumerate}
\item fix the value $p_j$, $j=1,2$ in \eqref{eq2}	and get $\hat{\beta}_j$, $j=1,2$, for each time series $\{y_{jt},\,t=1,\ldots,T\}$;
\item evaluate the AIC-like criterion
$
AIC_j(m)=\sum_{t=1}^{T}\rho_{p}(y_{jt}-x_{t}'\hat\beta_j)+2 m
$;
\item repeat step 1 and 2 for each   statistical unit $i$ and obtain the value $AIC_j^{(i)}(m)$, $i=1,\ldots,n$;
\item find the value $m$ that minimizes the overall  value
%\begin{equation}\label{eq:overall_AIC}
$\overline{AIC}(m)=\sum_{i=1}^n\sum_{j=1}^2 AIC_j^{(i)}(m)$.
%\end{equation}
\end{enumerate}	
In our simulation study  we consider the median value for both  time series, i.e. $p_1=p_2=0.5$.

For estimating the model parameters $\boldsymbol{\psi}$, we run  the MCMC for $100$ iterations as burn-in and $300$ iterations for getting the posterior estimates. Inspection of trace plots suggests convergence of the parameters. 
 From the clustering partitions sampled in the MCMC algorithm we obtain an estimate of the clustering structure by considering the posterior mode.


Both experiments are repeated  $100$ times.  We compared the performance of our clustering method with three state-of art competitors:
\begin{itemize}
	\item [1)] Gaussian finite Mixture model Clustering (GMC): we cluster the data by means of a mixture of Gaussian linear regression models. For estimating the parameter we exploit the R package \texttt{flexmix} \citep{flexmix} which is based on Expectation-Maximization  algorithm;
	% We clustered the bivariate time series using two independent splines regression with 4 basis of splines. 
	\item [2)] Raw Data Clustering (RDC): each bivariate time series is stacked in one vector. Then the vectors are clustered by means of a Partitioning Around Medoids (PAM) algorithm, extracting three clusters;
	\item[3)] CHaracteristic-based Clustering (CHC). A global measure describing the time series is obtained by applying summary indices about trend, seasonality, periodicity, serial correlation, skewness, kurtosis, chaos, nonlinearity and self-similarity \citep{Wang2006}. The normalized indices or features extracted by  using the R package \texttt{tsfeatures} \citep{tsfeatures}
	 are the inputs of the PAM algorithm. 
	
\end{itemize}

We assess the power of our clustering algorithm in reconstructing the three clusters by comparing the level of agreement between the estimated partition and the true clustering using 
the Adjusted Rand Index, ARI, \citep{Hubert1985}.

 Table \ref{bivsimARI} presents the ARI values for the combinations of the correlation structures and the marginal distribution.
From these results we note that our bivariate clustering algorithm performs very well at the combination, reporting low clustering performance for the more complex structure in particular for $\phi$=0.5; the simulation with the Gamma distribution (Sim B) appears more challenging in the clustering for all the considered methods.  It is worth to note that our method reported a better classification than the Gaussian mixed linear regression model even in the case of normal marginal distribution, especially in presence of a serial dependence.

\begin{table}[h!]\centering\vspace{0.5cm}
	\arrayrulecolor{black}
	\medskip
	\begin{tabular}{lcccccc}
		\hline
			 &$\rho$&$\theta$& {Our method} & GMC & RDC & CHC  \\
		\hline
		Sim A	&	$0$&$0 $ & $ 1.00\, (0.01) $ & $ 0.94\, (0.10) $& $ 1.00\, (0.01) $& $ 0.82\, (0.08) $\\
		&	$ 0.5$&$0  $ & $ 1.00\, (0.01) $ & $ 0.95\, (0.09) $& $ 1.00\, (0.01) $& $ 0.80\, (0.05) $\\
		
		&	$ 0.5$&$1.0  $ & $ 0.91\, (0.15) $ & $ 0.57\, (0.06) $& $ 0.75\, (0.09) $& $ 0.57\, (0.07) $\\
		\hline
		Sim B	&	$ 0$&$0 $ & $ 0.84\,(0.12) $ & $ 0.44\, (0.05)  $& $ 0.35\, (0.11) $& $ 0.55\, (0.09) $\\
		&	$ 0.5$&$0  $ & $ 0.56\, (0.29)  $ & $ 0.44\, (0.05) $& $ 0.35\, (0.10) $& $ 0.58\, (0.06) $\\	
		&	$ 0.5$&$1.0  $ & $ 0.32\, (0.22) $ & $ 0.32\, (0.05) $& $ 0.22\, (0.10)  $& $ 0.42\, (0.06) $\\
		\hline
	\end{tabular}
	\caption{Average (standard error between parentheses) Adjusted Rand Index values of 100 replications for each $\rho$ and $\theta$  combination, marginal distribution and clustering method.\label{bivsimARI}}

\end{table}



==> data.tex <==
\section{Chl-a and KD-490 levels in the Gulf of Gabes}\label{sec2}
The Gulf of Gabes is a Mediterranean zone with important biological resources and rich coastal, marine and freshwater ecosystems. In the last decades the Gulf of Gabes reported several environmental problems mainly due to the presence of human activities associated with over-fishing and seabed trawling while the presence of chemical factories in the Sfax site resulting on a wide wastewater pollution \citep{Aloulou:2012,Rabaoui:2013,Zaghden:2014,Fourati:2018}.
The results had led  to  several issues as the local appearance of red tides \citep{hamza:1994} as well as the changes or decline of the distribution of some marine species \citep{el:2016,el:2018}.

The European Community indicates  the diffuse Chlorophyll type-a (Chl-a) concentrations as a trophic status indicator of the sea-water. High Chl-a levels may lead to hypoxic or anoxic events.  KD-490 indicates how the solar light can penetrate to deeper water and can be used to evaluate the potential disturbance to the water ecosystem.

In this work, we considered two datasets comprising the Chl-a concentrations and the KD-490 levels made available by ACRI (\texttt{hermes.acri.fr}) in the framework of the GlobColour Project (\texttt{www.globcolour.info}).
The datasets were formed by monthly values of Chl-a concentrations and KD-490 levels in the Gulf of Gabes from January, 2003 to December, 2011 for a total of $108$ time-points.
Data were obtained by calibrating Ocean Colour data provided by different satellite missions, such as MERIS, SeaWiFS and MODIS. For each month, gridded data with 1.8-km resolution are available and  a  grid of $4,033$ points  covers the entire Gulf of Gabes.

%%%decribe the tow figures 
In Figure \ref{fig:1} we report the average levels of Chl-a concentration and KD-490 index for all the sites.
% describe the temporal trend of the selected sites.
%%%%%%%%%%%%%%%

\begin{figure}
	\centering
	\begin{tabular}{cc}
		\includegraphics[width=0.5\linewidth]{meanChla_trim.png}  &
		\includegraphics[width=0.5\linewidth]{meanKD490_trim.png} \\
		%(a) & (b)
	\end{tabular}
	\caption{Observed grid-points (4033 sites) in the Gulf of Gabes for Chl-a (left) and KD-490 (right) and two example sites reported in Figure \ref{fig:2}.}\label{fig:1}
\end{figure}
The highest average levels of Chl-a and KD-490 were reported near the coastal area, in the north-eastern zone (Sfax) and in the southern part (Djerba) of the Gulf. The spatial distribution of the average values between Chl-a and KD-490 appears to have a similar spatial and temporal behaviour, but not everywhere. In fact as shown in Figure \ref{fig:2} the example site 1 exhibits a strong seasonal pattern both in the Chl-a and KD-490 indicators, with a strong correlation between the two time series (Pearson $\rho$: 66.1\%); in the second example site 2 there is a clear difference between the trend of the Chl-a concentration with respect to the KD-490 one as attested by a weak correlation (Pearson $\rho$: 30.7\%).

\begin{figure}
	\centering
	\begin{tabular}{cc}
		\includegraphics[width=0.5\textwidth]{example1.png}  &
		\includegraphics[width=0.5\textwidth]{example2.png} \\
		(1) Lat: 10.88; Long: 33.99 & (2) Lat: 11.08; Long: 34.86
	\end{tabular}
	\caption{Temporal trend of Chl-a and Kd-490 in the two selected example sites.}\label{fig:2}
\end{figure}

The dataset is affected by outliers due to measurement errors  (Chl-a concentration lower than 0.05 $mg/m^{-3}$: 1.0\%; KD-490 levels lower than 0.05 $m^{-1}$: 2.8\%) and by a  different amount of missing observations
% please verify how many observations are missing
(Chl-a: 19.1\%; KD-490: 1.8\%).

The presented dataset presents several features which makes the clustering task challenging: a strong seasonality and a high variability,  the presence of outliers and a non bell-shaped distribution. The proposed classification may help to assess the trophic status of this area combining the information provided by different temporal Chl-a and KD-490 levels.


==> discussion.tex <==
\section{Discussion}\label{sec6}
In this paper we have proposed a new model based clustering technique,  that is capable of handling asymmetric clusters with presence of outliers as well as considering different quantile levels of the observed data. Our clustering strategy is based on the finite mixture model theory where each component of the mixture of AL distributions, which constitutes of the density of bivariate random variables which are potentially correlated, is assumed to represent a cluster with the skewness parameter of AL distribution being used to directly model the quantiles of interest. Our proposed technique therefore adds on to the richness of the recent burgeoning of non-Gaussian approaches to model-based clustering.

As the AL distribution provides a direct link between the maximum likelihood theory and minimization of a quantile regression check loss function \citep[see][]{koenker1999goodness,yu2001bayesian}, we estimate the cluster specific  parameters, which are the parameters of the mixing AL distribution, through a Bayesian quantile regression approach. Following from \cite{Waldmann2015} we implement our bivariate clustering model that is based on Bayesian bivariate quantile regression. We note that due to the dependence in the constructed likelihood for the bivariate random variables there are no closed form available conditional posteriors for the model parameters. We therefore, introduce MH steps to estimate the parameters through MCMC.

In our simulation experiment we considered three clusters two of which are not distinctively different from each other. However, an evaluation of the power of our proposed algorithm in reconstructing the three groups indicates a good performance with respect to the other competitive methods. We have applied the procedure to time series observed from GlobColour data related to Chlorophyll type-a concentrations and KD-490 levels in order to identify homogeneous areas in the Gulf of Gabes with respect to the temporal behavior of these water indicators. We defined clusters that are similar by different combination of quantiles of the two indicators. It is important to note that as different choice of quantiles implies changes in the clustering, this method may be particularly suitable for defining areas at different risk when considering two indicators at different quantile levels. More particularly, important features are of absolute interest in environmental sciences and ecology. \citep{schmidt2012estimating}.

We note that both Chl-a concentrations and KD-490 levels are affected by several spatially varying factors. Therefore, a potential future development of this work is to model spatial dependence for the time series observed at different spatial sites. This could be achieved either through Markov random fields that considers the nearest neighbors \citep{Gaetan:2017,jiang2012clustering}. By borrowing information from neighboring observation sites, this could lead to more smooth clusters. Another possible extension is to perform clustering at multiple quantiles instead of fixing the levels of quantiles. However, caution has to be taken in this case to avoid the issue of crossing quantiles.


==> methods.tex <==
\section{Statistical modelling and inference}\label{sec3}
 \subsection{Multivariate quantile regression and asymmetric Laplace distribution}
We start by considering the  univariate case.
 Let $ Q_{p}(y|x) $, for $ 0<p<1 $, be the $p$-th quantile regression function of the univariate continuous random variable $ y $ given $ x$, a vector of  covariates.
 We suppose that $ Q_{p}(y|x)=x'\beta $, where $ \beta $ is a vector of unknown parameters to be estimated. Then a quantile regression model can be defined as $y=x'\beta+e$
where $ e$ is an error term  with  density function $f(\cdot;p) $ and  the $ p $-th quantile equal to zero, i.e. $ \int_{-\infty}^{0}f(e;p)de=p$.
Owing to the data $(y_t,x_t')$, $t=1,\ldots, T$, the  estimate of $\beta$ is classically \citep{koenker1978regression} obtained by minimizing 
\begin{eqnarray}\label{eq2}
	\hat{\beta}=\underset{\beta}{\text{argmin}}\sum_{t=1}^{T}\rho_{p}(y_{t}-x_{t}'\beta),
\end{eqnarray}
where $ \rho_{p}(\cdot) $ is the check loss function, i.e. $ \rho_{p}(z)=z(p-I(z<0)) $.

\citet{koenker1999goodness} showed that there is a direct relationship between minimizing (\ref{eq2}) and the maximum likelihood theory using independent variables $y_t$ with  Asymmetric Laplace   (AL) density
\begin{equation}
	f(e;p)=\frac{p(1-p)}{\sigma}\exp\left\{-\rho_{p}\left(\frac{e}{\sigma}\right)\right\},\label{eq3}
\end{equation}
where $ \sigma>0 $  is an additional   scale parameter.

In the following we will exploit the representation of $y$ with density \eqref{eq3} as a location scale mixture of Gaussian random variable  \citep{Kotz2001}, namely
\begin{eqnarray}
	y=x'\beta+\theta \sigma w+\omega \sigma\sqrt{ w}\,\nu \label{eq5}
\end{eqnarray}
where $ \nu\sim \mathcal{N}(0,1) $, and $ w $ is a exponential random variable with  $E(w)=1$. Here $\nu $ and $ w $ are mutually independent and
$\theta=(1-2p)/\{p(1-p)\}$ and $\omega^{2}=2/\{p(1-p)\}$.


The literature has focused on univariate response variable with only a few studies considering extension to multivariate case \citep{Benoit2012,Benoit2013,Waldmann2015,Petrella2019a}.


In particular \cite{Petrella2019a} considered a multivariate  asymmetric Laplace distribution \citep{Kotz2001} to specify a quantile regression model for the random vector
$\tilde{y}=(y_1,\ldots,y_q)'$ in the mixture representation
\begin{equation}
	\tilde{y}=X'\tilde{\beta}+ D\Theta {w} +\sqrt{w}D\Sigma^{1/2}\tilde{\nu} \label{eq3.20}
\end{equation}

Here  $\tilde{\nu}$ denotes a $q$-dimension standard Gaussian vector and $w$ is a exponential random variable with unit mean.
The matrix $X$ is a $q\times L$  regressor matrix and $\tilde\beta$ is a $L$-dimensional unknown vector. The other parameters of the model are contained in  $D = \operatorname{diag}(\tilde\sigma)$, with $\tilde{\sigma}=(\sigma_1,\ldots,\sigma_q)'$,  $\sigma_j>0$, $j=1,\ldots,q$  and $\Theta= \operatorname{diag}(\theta_1,\ldots,
\theta_q)'$ with $\theta_j = (1 - 2p_j)/[p_j (1 - p_j]$. 

Moreover the matrix $\Sigma=\Omega R(\tilde\phi)\Omega$ is a $q \times q$ positive definite matrix   with $R(\tilde\phi)$ being a correlation matrix, that depends on a vector of parameters $\tilde\phi$, and $\Omega= \operatorname{diag}(\omega_1^2,\ldots,\omega_q^2)$,
with entry $\omega_{j}^{2}={2}/[p_{j}(1-p_{j})]$. Note that using this formulation the component $y_j$ will  always be mutually dependent, even though $R(\phi)$ is an identity matrix.

In this paper we  consider a slight different approach with respect to  \eqref{eq3.20}.
We use the same idea as in \cite{Waldmann2015} and we set

\begin{equation}\label{eq:ald}
	\tilde{y}=X'\beta+ D\Theta \tilde{w} +{W}^{1/2}D\Sigma^{1/2}\tilde{\nu} 
\end{equation}
with $\tilde{w}= ({w}_1,\ldots,w_q)'$ and ${W}= \operatorname{diag}({w}_1,\ldots,{w}_q)$
allowing a different  exponential random variable with unit mean $ w_j$ for each component.


With this variation   model \eqref{eq:ald} does not define a proper multivariate asymmetric Laplace distribution as in \citet{Kotz2001}. However the model becomes more flexible and can cover the case of mutually independent components.
Now the challenge  lies in finding a multivariate density
for $\tilde{w}$, $	e(\tilde{w};\gamma)$, with marginal exponential distributions for the $w_j$ in order to guarantee that the marginal distributions for the response variables are still asymmetric Laplace. Here the parameter $\gamma$ is a generic dependence parameter.
%Therefore the multivariate density function of \eqref{eq:ald}
%\begin{eqnarray}
%	\textrm{ald}(\tilde{y}|\tilde{x},\beta,D,R(\phi),\gamma) 
%	&=&\int_{(0,\infty)^q} (2\pi)^{-q/2}|W^{{1}/{2}}\varSigma W^{{1}/{2}}|^{-{1}/{2}}\times \nonumber\\
%	&& \exp\left\{-\frac{1}{2}(\tilde{y}-X'\beta- D\Theta \tilde{w})'W^{-{1}/{2}}\varSigma^{-1}W^{-{1}/{2}}(
%	\tilde{y}-X'\beta- D\Theta \tilde{w})\right\}\times\nonumber\\
%	&& f(\tilde{w};\gamma)d\tilde{w}
%\end{eqnarray}

Several multivariate exponential distributions   have been proposed in the literature \citep[Ch. 47]{kotz:balakrishnan:johnson}.
\cite{Waldmann2015} adopt the simplest specification that the exponential variables are independent, i.e. $\gamma=0$.

In view of the bivariate real data example in this paper we exemplify our construction by using the bivariate density proposed by \cite{Downton1970}, namely
\begin{equation}\label{eq:downton}
	e(\tilde{w};\gamma)= \frac{1}{(1-\gamma)}\exp \left\{-\frac{1}{1-\gamma}\left(w_{1}+w_{2}\right)\right\}
I_{0}\left(\frac{2}{1-\gamma}\sqrt{\gamma w_{1}w_{2}}\right)
\end{equation}
where $ 0\le\gamma < 1 $
and $I_{0}(a)=\sum_{k=1}^{\infty}\frac{a^{2k}}{4^{k}(k!)^{2}}$ is the modified Bessel function of the first kind of order zero.
The value $\gamma$ represents the 
Pearson's product-moment correlation and $ \gamma=0 $ implies independence between the $w_1$ and $w_2$.
Coupling \eqref{eq:ald} with the density \eqref{eq:downton} we obtain a  flexible specification of a bivariate quantile regression model that covers the case of independence between  the components when $R(\phi)$ is an identity matrix and $\gamma=0$.




\subsection{Model-based clustering}\label{subsec:mixmod}
Suppose that we observe  data over $n$ statistical units and, for simplicity,  the same number $q\times T$  of values $y_{ijt}$,  $j=1,\ldots, q$, $t=1,\ldots,T$, for each statistical unit $i$, $i=1,\ldots,n$.
We collect the observations for each unit into the vector $\boldsymbol{y}_i = (\tilde{y}_{i1}',\ldots, \tilde{y}_{iT}')'$, with
$\tilde{y}_{it} = (y_{i1t},y_{i2t},\ldots y_{iqt})'$, $t=1,\ldots,T$.
The vectors  $\boldsymbol{y}_i$ are supposed to be independent.
The whole dataset will be denoted by $\mathcal{Y}=(\boldsymbol{y}_1,\ldots,\boldsymbol{y}_n)$.

Our statistical  problem is to cluster the $n$ statistical units, i.e. the sites,  into the clusters $\{1,\ldots,K\}$, $K\ll n$.
We follow a  mixture-model  approach \citep{mclachlan:peel:2000}  to clustering  according to which the cluster membership of the $i$th unit is represented by a latent random variable  ${c}_i \in \{1,\ldots,K\} $ , where $c_{i} = k$ indicates if the $i$-th units belongs to the cluster $k$. 

The memberships ${c}_i$, $i=1,\ldots,n$ are supposed independent and identically distributed  variables with 
$\Pr(c_{i} = k)=\alpha_k$, $ 0<\alpha_{k}<1 $, for all $k=1,\ldots,K$ and $ \sum_{k=1}^{K}\alpha_{k}=1 $.



Given the cluster membership,  $c_{i}$,  observations for the $i$-th unit are generated by the mixture model specified hierarchically, namely 

\noindent\textbf{the observation level}
\begin{equation}\label{eq:model}
		\tilde{y}_{it}|c_i,\tilde{w}_{it}\sim\mathcal{N}_q(X_{t}'\tilde\beta_{c_i}+ D_{c_i}\Theta \tilde{w}_{it},{W}_{it}D_{c_i}\Sigma_{c_i}D_{c_i}{W}_{it}), \qquad i=1,\ldots,n,\quad t=1,\ldots,T 
\end{equation}
		conditionally independent distributed, with $\Sigma_{c_i}=\Omega R(\phi_{c_i})\Omega$;

\noindent \textbf{the latent process level}
\begin{equation}
		\tilde{w}_{it}|c_i\sim e(w,\gamma_{c_i}), \quad i=1,\ldots,n,\quad t=1,\ldots,T
\end{equation}
		conditionally independent distributed
\begin{equation}
		c_i \sim \operatorname{Multinomial}(1,{\alpha}), \quad i=1,\ldots,n
\end{equation}
independent distributed.  


\subsection{Bayesian inference}\label{subsec:bayinf}
We adopt a Bayesian approach to make inference on the model parameters.
The inference is facilitated by the fact that the mixture model is  specified hierarchically. Moreover
the conjugacy of some priors leads to  updates with
simple and established methods for drawing from the full
conditional distribution.
%Moreover it is possible to get the posterior probability of membership of a single vector, $\Pr(c_i=\cdot|\mathcal{Y})$.


\noindent \textbf{Prior distributions}

A common choice for the prior distribution of $\alpha$ is $ {\alpha}\sim \mathcal{D}(a_{1},...,a_{K}) $, where $\mathcal{D}$ is the Dirichlet distribution with parameters $a_1, \ldots, a_K > 0$;  % which is a conjugate prior for the mixing proportions

The choice $ \tilde\beta_{k} \sim \mathcal{N}(b_k,P_k),\, k=1,\ldots,K$, identically and independent distributed is still common and simplifies the simulation. Setting $ b_k=0 $ and $ P_k=a\,I $, for $ a \gg 0 $, leads to an improper prior.
		
		 Specification of the  prior distributions for
		$\tilde\sigma_1,\ldots,\tilde\sigma_k$ and $\tilde\phi_1,\ldots,\tilde\phi_k$  is complicated  by the complex requirement that the matrices $D_k\Omega R(\phi_{k})\Omega D_k$ are  non-negative definite matrices.
We follow \citet{barnard:mcculloch:meng:2000} and   work  by specifying prior for variances  and correlation matrices.
For the variances we put the priors $ \sigma^2_{kj} \sim \mathrm{IG}(s_{k},d_{k}),\quad k=1,\ldots,K,\quad j=1,\ldots,q$,  identically and independent distributed,
	where $IG$ is  the inverse gamma distribution,
	with the shape $ s_{k}$  and $ d_{k}$ scale parameters.
	\citet{barnard:mcculloch:meng:2000} discussed the relative merits of choosing a prior for $\tilde\phi_1,\ldots,\tilde\phi_k$ independent from $\tilde\sigma_1,\ldots,\tilde\sigma_k$.
 In our example the choice is greatly simplified since we consider two variables, i.e. $q=2$. In that case
we can assign assign a uniform prior, $\phi_k\sim\mathcal{U}(-1,1)$,  for the correlation coefficient $\phi_k$ that are supposed identically and independent distributed.
	


For sampling
from the posterior distribution we use a hybrid MCMC algorithm known as Metropolis-within-Gibbs algorithm \citep[][Chapter 10]{Robert2004}.
As we show in the Supplementary material the conjugacy of some priors leads to  updates with
simple, established methods for drawing from the full
conditional distribution.
In other cases, we  resort to Metropolis-Hastings
to draw from some of the full conditional distributions.




==> results.tex <==
\section{Clustering sites in the Gulf of Gabes}\label{sec5}

In this section we present the clustering results for the bivariate variables Chl-a concentration and the KD-490 levels, previously presented in Section \ref{sec2}.  
As reported in Figure \ref{fig:2}, we can observe a strong and time-varying seasonal pattern, with the presence of a peak at the beginning of each year. For this reason
 we choose to model such monthly seasonality using sine and cosine functions \citep{eilers2008modulation}.
 More precisely we suppose that for each variable $y$ the quantile regression function is a function of the time $t$, such that 
 \begin{equation*}%\label{eq5.bis}
Q_p(y|t)=g_1(t)+ g_2(t) \cos(\pi/6t)+ g_3(t) \sin(\pi/6t)
 \end{equation*}
 where   a possible overall trend is represented by a smooth function $g_1(t)$, while $g_2(t)$ and $g_3(t)$ are smooth functions  that modulate the local amplitudes of the cosine and sine waves. 

In order to have a good grade of flexibility, the three  functions $g_1(t)$, $g_2(t)$, and $g_3(t)$ take the form of a regression on a cubic B-spline basis, $
g_j(t)= \sum_{l=1}^{m_j} \beta_{jl} b_l(t)
$
with  equally spaced knots over the time interval $[1,108]$.
It is easy to see that the resulting  model for the quantile function
 \begin{equation*}%\label{eq5.bis}
	Q_p(y|t)=\sum_{l=1}^{m_1} \beta_{1l} b_l(t)+ \sum_{l=1}^{m_2} \beta_{2l}[b_l(t)\cos(\pi/6t)]+ \sum_{l=1}^{m_3} \beta_{3l}[b_l(t)\sin(\pi/6t)]
\end{equation*}
can be written as a linear combination of covariates  that fits with \eqref{eq:ald}.

We carry out a preliminary data analysis in order to get the degree of smoothing and the number of clusters.
This data  analysis has been performed on the time series  of Chl-a concentration since this variable displayed more heterogeneity in space and time.


To find the  grade of smoothing and obtain a value for $m_1$, $m_2$, and $m_3$, we follow the strategy outlined in Section \ref{sec4} and we minimize the overall value $AIC(m)$, with  $m=m_1+m_2+m_3$  by means of a median (i.e. $p=0.5$) regression.  
The solution with $m_1=4$ for the  trend (with the inclusion of a internal intercept) and $m_2=m_3=3$ for the cyclical components minimized the overall $AIC(m)$ and it was chosen  in the model.
Having fixed the number of covariates and still fixing $p=0.5$ we  identify the number of clusters, $K=5$ by minimizing  the  conditional version named $DIC_8$ \citep{celeux2006deviance} of
Deviance Information Criteria \citep{spiegelhalter2002bayesian}.

Then we fit a bivariate model assuming that the two time series have a constant correlation coefficient across the clusters, i.e. $\phi=\phi_k$.
Moreover a word of caution is in order of the estimate of the parameter $\gamma$ in \eqref{eq:downton}. Our experience with this dataset indicates that the the data provide very little information on the parameter. For this reason we set the value $\gamma=0.5$,
giving the parameter $\phi$ the task of modulating the dependence 
between the two time series.

 We estimate the model for a range of different quantile combinations namely for different values of $(p_{1},p_{2})$. Particularly we consider the combination of quantiles given by the pairs $ (0.5,0.5) $, $ (0.9,0.5) $, and $ (0.9,0.9) $ for Chl-a concentration and KD-490, respectively.

The results were obtained after 2500 Monte Carlo iterations using a burn-in of 200. The final membership ${c}_i$ and the regression coefficients $\beta_{jl}$ were estimated by means of the mode and mean of a-posteriori distribution, respectively. In Figure \ref{spatial} we present the spatial distribution of the clustering results for each combination quantiles.



Across all the fitted quantile combinations, we observe that those regions around the islands (Kerkennah, Kneiss and Jerba) are clustered as having the highest average values of both Chl-a and KD-490 concentration which decreases as one moves towards the deep sea. These results are consistent with the results obtained from the univariate case as well as the findings of \cite{Katlane2012} who notes that, from multi-temporal turbidity maps produced from Moderate Resolution Imaging Spectrometer (MODIS) for $ 2009 $, areas around the islands (Kerkenah, Kneiss and Jerba) and at the industrial port of Gannouch, were characterized by high turbidity variation, concentration of total suspended matter and Chl-a concentration.

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{spatial_results.png}
	\caption{Spatial clustering results for Chl-a concentration and KD-490 index at quantile combination (a) $ (0.5,0.5)$, (b) $ (0.9,0.5)$, and (c) $ (0.9,0.9). $\label{spatial} }
\end{figure}

However, given the different meaning of Chl-a concentration and KD-490 levels at each quantile level, the spatial distribution between the three classifications appears different in particular looking to the northeastern area and to coastal zone. In fact the classification with (0.5,0.5) identifies a series of clusters which describe not only the most polluted area (Cluster $4$ and $5$), but also the coastal area (Cluster $3$) and the zone inside the Gulf (Cluster $2$). Otherwise, the classification in (0.9,0.5) and  (0.9,0.9) reported a wide cluster $1$ which covers a zone starting from the offshore waters to the coastal area, with the exception of the islands and the Sfax industrial area in the north-east.  In fact, as reported in Figure \ref{boxplots}, the classification performed with the quantile combination (0.5, 0.5) reported an increasing trend of both Chl-a concentration and KD-490 levels. The clustering performed with a quantile combination of 0.9 for Chl-a and 0.5 for KD-490 appears different with respect to the combination $(0.5,0.5)$ both in terms of group size and the median values across clusters: cluster $1$ embraces the 88.6\% of the sites and the Chl-a values of the cluster $2$ and $3$ overlapped as well as those of the cluster $4$ and $5$; low KD-490 levels are restricted to the cluster $1$ while the cluster $4$ reports the highest one. In the classification with the quantile combination $(0.9,0.9)$, the number of sites which belongs to cluster $1$ increases (94.4\%) while cluster $3$ and $4$ are represented by only 3 and 8 sites, respectively. The Chl-a values in the cluster $1$ are low and well separated by the cluster $2$ and $5$; the KD-490 levels of the cluster $2$ and $5$ are similar. The meaning of the classification with the quantile combination $(0.9,0.9)$ is similar to those of the previous classification $(0.9, 0.5)$, but with a greater spatial continuity among the cluster membership.
For both the  classifications with the quantile combination $(0.9, 0.9)$ and $(0.9,0.5)$, especially the last, some clusters are represented by a low number of sites indicating that a lower number of cluster may be more appropriate.


\begin{figure}[h!]
	\centering
	\includegraphics[width=1\textwidth]{boxplots.png}\\
	\caption{Distribution of Chl-a concentration and KD-490 index by Cluster fo each quantile combination (a) $ (0.5,0.5) $, (b) $ (0.9,0.5)$ and  (c) $ (0.9,0.9). $\label{boxplots} }
\end{figure}

In Figure \ref{timeseries} the temporal pattern for each recovered cluster is reported by plotting the estimated quantile functions  of Chl-a concentration and KD-490 for each considered combination of quantiles. For all cluster a seasonal pattern is evident. Cluster labels and colors are the same as those in Figure \ref{spatial}. %and they are ordered by average $\hat{g(t)}$ of the Chl-a value. 
The classification with the quantile combination $(0.5,0.5)$ is guided by different average levels in Chl-a concentration with the last cluster looking different from the others; the clustering on KD-490 identifies five clusters with different average values and denotes an increasing trend for the Clusters $4$ and $5$ at the beginning of the time window followed by an increasing oscillation.
Considering the clustering results obtained by the quantile combination $(0.9-0.5)$, the temporal trend appears different with respect to the previous classification: Clusters from $2$ to $5$ reported an increasing trend and a stabilization after 2007 for both Chl-a and KD490 indicators; the seasonal component appears more evident in the quantile 0.5 of KD-490 levels than in the quantile 0.9 of the Chl-a concentration; Chl-a concentration of Clusters $4$ and $5$ appears to be similar in average, but the oscillation in the Cluster $5$ is smoothed. For the KD-490, Cluster $4$ reports the highest level, followed by Cluster $5$ and then by $3$ and $2$, very close to each other. The Cluster $1$ showed the lowest values and a wide distance from the other groups for both the indicators. The clustering of the quantile combination $(0.9-0.9)$ shows: an increasing trend and a stabilization after 2007 only for the Chl-a concentration for the Clusters $2$, $3$, and $5$; Clusters from $2$ to $5$ report a similar behaviour; with the exception of the first cluster, KD-490 levels are similar among the identified pair of Clusters $5$ and $2$, and $3$ and $4$, with a decreasing amplitude in the cluster $4$. For both the indicators Cluster $1$ reports values far from the other groups.

\newpage
\begin{figure}[h!]
	\centering
%	\text{(a)}
	\includegraphics[height=0.3\textheight]{time_series0505.png}\\
%	\text{(b)}
	\includegraphics[height=0.3\textheight]{time_series0905.png}\\
%	\text{(c)}
	\includegraphics[height=0.3\textheight]{time_series0909.png}\\
	\caption{Average quantiles for Chl-a concentration and KD-490 index at several combinations of percentages $(p_1,p_2)$.  $ (0.5,0.5)  $ (top),  $ (0.9,0.5)$ (middle), and   $ (0.9,0.9) $ (bottom). \label{timeseries} }
\end{figure}

